Sequential Semantic-Non-Semantic Watermarking: Robustness Against UnMarker Attacks

Advancements in artificial intelligence (AI) have accelerated digital content generation and intensified concerns around fraud, misuse, counterfeiting, and content provenance. Defensive image watermarking provides a practical mechanism for identifying and tracing digital content, but recent watermark-removal attacks challenge its robustness. This study investigates Sequential Semantic Non-Semantic Watermarking (SSNSW), which combines HiDDeN and StegaStamp as complementary non-semantic and semantic watermarking schemes. Using 50 images from MS-COCO and CelebA-HQ, both embedding orders are evaluated, followed by UnMarker's non-semantic and semantic attacks applied individually and sequentially. Results show that both watermarks remain highly decodable after dual embedding, with only limited embedding-order effects. Under individual attacks, one watermark generally remains strongly decodable: StegaStamp under the non-semantic attack and HiDDeN under the semantic attack. Sequential attacks are therefore required to substantially reduce both watermark signals, while attack order has a limited and configuration-dependent effect. The semantic attack also shows a broader effect across the two watermark types than the non-semantic attack. LPIPS remains relatively low in several settings, although qualitative inspection reveals noticeable distortions, particularly in selected facial images, indicating that LPIPS should not be used alone to assess visual quality. Overall, the findings show that combining complementary watermark types can increase robustness against single-stage removal attacks and motivate broader multi-layer watermarking, stronger perceptual evaluation, and further study of sequential watermark-removal strategies.

==> appendices/detailed_experimental_results.tex <==
\section{Appendix - Detailed experimental results} \label{chap: Detailed Experimental Results}
\subsection{Phase 1: Baseline study}
\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lcccc}
\caption{Base HiDDeN attacked by \textbf{non-semantic attack}: per-image bit accuracy before watermarking ($\mathrm{BA}_{\text{orig}}$), after watermarking ($\mathrm{BA}_{\text{wm}}$), and after removal ($\mathrm{BA}_{\text{att}}$), with similarity score. Images 1--25: COCO, 26--50: CelebA.}
\label{tab:hidden_base_nonsemantic}\\
\toprule
Image & $\mathrm{BA}_{\text{orig}}$ & $\mathrm{BA}_{\text{wm}}$ & $\mathrm{BA}_{\text{att}}$ & Similarity Score \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{orig}}$ & $\mathrm{BA}_{\text{wm}}$ & $\mathrm{BA}_{\text{att}}$ & Similarity Score \\
\midrule
\endhead

\midrule
\multicolumn{5}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1  & 0.630 & 1.000 & 0.600 & 0.065 \\
image\_2  & 0.570 & 1.000 & 0.470 & 0.092 \\
image\_3  & 0.500 & 1.000 & 0.500 & 0.074 \\
image\_4  & 0.700 & 1.000 & 0.600 & 0.042 \\
image\_5  & 0.600 & 1.000 & 0.570 & 0.038 \\
image\_6  & 0.430 & 1.000 & 0.570 & 0.083 \\
image\_7  & 0.600 & 1.000 & 0.500 & 0.058 \\
image\_8  & 0.630 & 1.000 & 0.600 & 0.046 \\
image\_9  & 0.630 & 1.000 & 0.530 & 0.087 \\
image\_10 & 0.570 & 1.000 & 0.570 & 0.099 \\
image\_11 & 0.530 & 1.000 & 0.530 & 0.051 \\
image\_12 & 0.670 & 1.000 & 0.530 & 0.092 \\
image\_13 & 0.530 & 1.000 & 0.600 & 0.063 \\
image\_14 & 0.500 & 1.000 & 0.500 & 0.069 \\
image\_15 & 0.630 & 1.000 & 0.530 & 0.057 \\
image\_16 & 0.630 & 1.000 & 0.530 & 0.064 \\
image\_17 & 0.570 & 1.000 & 0.600 & 0.068 \\
image\_18 & 0.530 & 1.000 & 0.570 & 0.081 \\
image\_19 & 0.470 & 1.000 & 0.570 & 0.070 \\
image\_20 & 0.500 & 1.000 & 0.530 & 0.079 \\
image\_21 & 0.570 & 1.000 & 0.470 & 0.065 \\
image\_22 & 0.700 & 1.000 & 0.530 & 0.071 \\
image\_23 & 0.600 & 1.000 & 0.530 & 0.087 \\
image\_24 & 0.630 & 1.000 & 0.600 & 0.066 \\
image\_25 & 0.600 & 1.000 & 0.600 & 0.092 \\
image\_26 & 0.600 & 1.000 & 0.530 & 0.138 \\
image\_27 & 0.570 & 1.000 & 0.400 & 0.129 \\
image\_28 & 0.430 & 1.000 & 0.570 & 0.109 \\
image\_29 & 0.570 & 1.000 & 0.670 & 0.055 \\
image\_30 & 0.700 & 1.000 & 0.600 & 0.050 \\
image\_31 & 0.600 & 1.000 & 0.600 & 0.080 \\
image\_32 & 0.470 & 1.000 & 0.530 & 0.096 \\
image\_33 & 0.570 & 1.000 & 0.570 & 0.070 \\
image\_34 & 0.430 & 1.000 & 0.500 & 0.139 \\
image\_35 & 0.670 & 1.000 & 0.630 & 0.086 \\
image\_36 & 0.530 & 1.000 & 0.530 & 0.082 \\
image\_37 & 0.630 & 1.000 & 0.630 & 0.085 \\
image\_38 & 0.600 & 1.000 & 0.530 & 0.107 \\
image\_39 & 0.700 & 1.000 & 0.630 & 0.028 \\
image\_40 & 0.470 & 1.000 & 0.470 & 0.147 \\
image\_41 & 0.570 & 1.000 & 0.670 & 0.031 \\
image\_42 & 0.670 & 1.000 & 0.570 & 0.072 \\
image\_43 & 0.600 & 1.000 & 0.470 & 0.060 \\
image\_44 & 0.600 & 1.000 & 0.600 & 0.042 \\
image\_45 & 0.630 & 1.000 & 0.700 & 0.062 \\
image\_46 & 0.630 & 1.000 & 0.630 & 0.049 \\
image\_47 & 0.530 & 1.000 & 0.600 & 0.037 \\
image\_48 & 0.670 & 1.000 & 0.470 & 0.097 \\
image\_49 & 0.570 & 1.000 & 0.500 & 0.073 \\
image\_50 & 0.600 & 1.000 & 0.570 & 0.113 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.581 & 1.000 & 0.549 & 0.070 \\
\textbf{Average (CelebA, 26--50)} & 0.584 & 1.000 & 0.567 & 0.082 \\

\end{longtable}
\endgroup



\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lcccc}
\caption{Base StegaStamp attacked by \textbf{semantic attack}: per-image bit accuracy before watermarking ($\mathrm{BA}_{\text{orig}}$), after watermarking ($\mathrm{BA}_{\text{wm}}$), and after removal ($\mathrm{BA}_{\text{att}}$), with similarity score. Images 1--25: COCO, 26--50: CelebA.}
\label{tab:stega_base_semantic}\\
\toprule
Image & $\mathrm{BA}_{\text{orig}}$ & $\mathrm{BA}_{\text{wm}}$ & $\mathrm{BA}_{\text{att}}$ & Similarity Score \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{orig}}$ & $\mathrm{BA}_{\text{wm}}$ & $\mathrm{BA}_{\text{att}}$ & Similarity Score \\
\midrule
\endhead

\midrule
\multicolumn{5}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1  & 0.490 & 1.000 & 0.640 & 0.055 \\
image\_2  & 0.520 & 1.000 & 0.550 & 0.089 \\
image\_3  & 0.470 & 1.000 & 0.560 & 0.060 \\
image\_4  & 0.510 & 1.000 & 0.670 & 0.059 \\
image\_5  & 0.520 & 1.000 & 0.580 & 0.048 \\
image\_6  & 0.580 & 1.000 & 0.510 & 0.060 \\
image\_7  & 0.550 & 1.000 & 0.660 & 0.055 \\
image\_8  & 0.580 & 1.000 & 0.560 & 0.073 \\
image\_9  & 0.450 & 1.000 & 0.630 & 0.074 \\
image\_10 & 0.530 & 1.000 & 0.600 & 0.072 \\
image\_11 & 0.470 & 1.000 & 0.690 & 0.052 \\
image\_12 & 0.510 & 1.000 & 0.580 & 0.078 \\
image\_13 & 0.500 & 0.990 & 0.620 & 0.060 \\
image\_14 & 0.510 & 1.000 & 0.590 & 0.057 \\
image\_15 & 0.390 & 1.000 & 0.620 & 0.062 \\
image\_16 & 0.510 & 1.000 & 0.570 & 0.066 \\
image\_17 & 0.460 & 1.000 & 0.620 & 0.063 \\
image\_18 & 0.460 & 1.000 & 0.530 & 0.068 \\
image\_19 & 0.410 & 1.000 & 0.650 & 0.081 \\
image\_20 & 0.550 & 1.000 & 0.520 & 0.092 \\
image\_21 & 0.540 & 1.000 & 0.540 & 0.071 \\
image\_22 & 0.470 & 1.000 & 0.630 & 0.058 \\
image\_23 & 0.450 & 0.990 & 0.600 & 0.066 \\
image\_24 & 0.440 & 0.990 & 0.690 & 0.065 \\
image\_25 & 0.530 & 1.000 & 0.630 & 0.080 \\
image\_26 & 0.550 & 1.000 & 0.510 & 0.100 \\
image\_27 & 0.460 & 1.000 & 0.600 & 0.094 \\
image\_28 & 0.510 & 1.000 & 0.670 & 0.075 \\
image\_29 & 0.450 & 1.000 & 0.610 & 0.041 \\
image\_30 & 0.470 & 1.000 & 0.480 & 0.062 \\
image\_31 & 0.530 & 1.000 & 0.630 & 0.067 \\
image\_32 & 0.550 & 1.000 & 0.460 & 0.097 \\
image\_33 & 0.500 & 1.000 & 0.550 & 0.064 \\
image\_34 & 0.530 & 1.000 & 0.560 & 0.106 \\
image\_35 & 0.570 & 1.000 & 0.580 & 0.090 \\
image\_36 & 0.560 & 1.000 & 0.590 & 0.054 \\
image\_37 & 0.530 & 1.000 & 0.560 & 0.086 \\
image\_38 & 0.500 & 1.000 & 0.650 & 0.075 \\
image\_39 & 0.490 & 1.000 & 0.550 & 0.034 \\
image\_40 & 0.530 & 1.000 & 0.660 & 0.102 \\
image\_41 & 0.500 & 1.000 & 0.590 & 0.044 \\
image\_42 & 0.590 & 1.000 & 0.490 & 0.072 \\
image\_43 & 0.540 & 1.000 & 0.600 & 0.058 \\
image\_44 & 0.540 & 1.000 & 0.520 & 0.057 \\
image\_45 & 0.560 & 1.000 & 0.520 & 0.051 \\
image\_46 & 0.500 & 1.000 & 0.540 & 0.061 \\
image\_47 & 0.560 & 1.000 & 0.600 & 0.048 \\
image\_48 & 0.540 & 1.000 & 0.460 & 0.109 \\
image\_49 & 0.480 & 1.000 & 0.550 & 0.071 \\
image\_50 & 0.470 & 1.000 & 0.550 & 0.085 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.496 & 0.999 & 0.602 & 0.067 \\
\textbf{Average (CelebA, 26--50)} & 0.520 & 1.000 & 0.563 & 0.072 \\

\end{longtable}
\endgroup

\subsection{Phase 2: Dual watermarking study}
\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lccc}
\caption{Phase 2 (HiDDeNStega) --- Step 1: HiDDeN embedding on the benchmark dataset. Per-image bit accuracy for each decoder: $\mathrm{BA}_{\text{HiDDeN}}$ and $\mathrm{BA}_{\text{Stega}}$, with similarity score. Images 1--25: COCO, 26--50: CelebA.}
\label{tab:phase1_hiddenstega_step1_hidden_embed}\\
\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & Similarity Score \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & Similarity Score \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1.png  & 1.000 & 0.530 & 0.026 \\
image\_2.png  & 1.000 & 0.560 & 0.073 \\
image\_3.png  & 1.000 & 0.430 & 0.039 \\
image\_4.png  & 1.000 & 0.500 & 0.026 \\
image\_5.png  & 1.000 & 0.530 & 0.024 \\
image\_6.png  & 1.000 & 0.520 & 0.059 \\
image\_7.png  & 1.000 & 0.570 & 0.024 \\
image\_8.png  & 0.970 & 0.610 & 0.041 \\
image\_9.png  & 1.000 & 0.500 & 0.046 \\
image\_10.png & 1.000 & 0.570 & 0.043 \\
image\_11.png & 1.000 & 0.420 & 0.027 \\
image\_12.png & 1.000 & 0.500 & 0.051 \\
image\_13.png & 1.000 & 0.570 & 0.028 \\
image\_14.png & 1.000 & 0.500 & 0.029 \\
image\_15.png & 1.000 & 0.470 & 0.033 \\
image\_16.png & 1.000 & 0.500 & 0.031 \\
image\_17.png & 1.000 & 0.430 & 0.034 \\
image\_18.png & 1.000 & 0.470 & 0.034 \\
image\_19.png & 1.000 & 0.450 & 0.044 \\
image\_20.png & 0.970 & 0.520 & 0.049 \\
image\_21.png & 1.000 & 0.570 & 0.036 \\
image\_22.png & 1.000 & 0.480 & 0.035 \\
image\_23.png & 1.000 & 0.420 & 0.038 \\
image\_24.png & 1.000 & 0.470 & 0.028 \\
image\_25.png & 1.000 & 0.480 & 0.049 \\
image\_26.png & 1.000 & 0.550 & 0.073 \\
image\_27.png & 1.000 & 0.540 & 0.089 \\
image\_28.png & 1.000 & 0.490 & 0.050 \\
image\_29.png & 1.000 & 0.490 & 0.068 \\
image\_30.png & 1.000 & 0.460 & 0.037 \\
image\_31.png & 1.000 & 0.500 & 0.041 \\
image\_32.png & 1.000 & 0.470 & 0.070 \\
image\_33.png & 1.000 & 0.570 & 0.037 \\
image\_34.png & 1.000 & 0.490 & 0.080 \\
image\_35.png & 1.000 & 0.540 & 0.062 \\
image\_36.png & 1.000 & 0.520 & 0.055 \\
image\_37.png & 1.000 & 0.580 & 0.041 \\
image\_38.png & 1.000 & 0.560 & 0.062 \\
image\_39.png & 1.000 & 0.500 & 0.034 \\
image\_40.png & 0.930 & 0.550 & 0.084 \\
image\_41.png & 0.970 & 0.550 & 0.028 \\
image\_42.png & 1.000 & 0.570 & 0.038 \\
image\_43.png & 1.000 & 0.530 & 0.040 \\
image\_44.png & 1.000 & 0.540 & 0.020 \\
image\_45.png & 1.000 & 0.600 & 0.040 \\
image\_46.png & 1.000 & 0.490 & 0.029 \\
image\_47.png & 0.970 & 0.500 & 0.028 \\
image\_48.png & 1.000 & 0.500 & 0.067 \\
image\_49.png & 1.000 & 0.520 & 0.077 \\
image\_50.png & 0.970 & 0.460 & 0.055 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.998 & 0.503 & 0.038 \\
\textbf{Average (CelebA, 26--50)} & 0.994 & 0.523 & 0.052 \\

\end{longtable}
\endgroup


\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lccc}
\caption{Phase 2 (HiDDeNStega) --- Step 2: StegaStamp embedding on the HiDDeN-embedded dataset to create \textit{HiDDeNStega}. Per-image bit accuracy for each decoder: $\mathrm{BA}_{\text{HiDDeN}}$ and $\mathrm{BA}_{\text{Stega}}$, with similarity score. Images 1--25: COCO, 26--50: CelebA.}
\label{tab:phase1_hiddenstega_step2_stega_embed}\\
\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & Similarity Score \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & Similarity Score \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1.png  & 1.000 & 0.980 & 0.141 \\
image\_2.png  & 0.930 & 0.980 & 0.199 \\
image\_3.png  & 0.970 & 0.990 & 0.131 \\
image\_4.png  & 1.000 & 0.980 & 0.128 \\
image\_5.png  & 1.000 & 0.980 & 0.120 \\
image\_6.png  & 0.930 & 0.980 & 0.157 \\
image\_7.png  & 1.000 & 0.980 & 0.105 \\
image\_8.png  & 0.930 & 0.980 & 0.077 \\
image\_9.png  & 1.000 & 0.980 & 0.133 \\
image\_10.png & 1.000 & 0.980 & 0.227 \\
image\_11.png & 1.000 & 0.980 & 0.143 \\
image\_12.png & 1.000 & 0.990 & 0.135 \\
image\_13.png & 0.970 & 0.980 & 0.122 \\
image\_14.png & 1.000 & 0.980 & 0.124 \\
image\_15.png & 0.870 & 0.980 & 0.156 \\
image\_16.png & 1.000 & 0.990 & 0.141 \\
image\_17.png & 1.000 & 0.980 & 0.122 \\
image\_18.png & 1.000 & 0.980 & 0.150 \\
image\_19.png & 1.000 & 0.980 & 0.108 \\
image\_20.png & 0.970 & 0.980 & 0.153 \\
image\_21.png & 0.970 & 0.980 & 0.117 \\
image\_22.png & 1.000 & 0.990 & 0.142 \\
image\_23.png & 0.900 & 0.980 & 0.226 \\
image\_24.png & 1.000 & 0.980 & 0.093 \\
image\_25.png & 0.970 & 0.980 & 0.200 \\
image\_26.png & 1.000 & 0.980 & 0.128 \\
image\_27.png & 1.000 & 0.980 & 0.092 \\
image\_28.png & 1.000 & 0.980 & 0.113 \\
image\_29.png & 1.000 & 0.980 & 0.109 \\
image\_30.png & 0.930 & 0.980 & 0.088 \\
image\_31.png & 1.000 & 0.980 & 0.069 \\
image\_32.png & 1.000 & 0.980 & 0.087 \\
image\_33.png & 0.970 & 0.980 & 0.116 \\
image\_34.png & 0.970 & 0.980 & 0.207 \\
image\_35.png & 1.000 & 0.980 & 0.114 \\
image\_36.png & 1.000 & 0.990 & 0.116 \\
image\_37.png & 1.000 & 0.980 & 0.117 \\
image\_38.png & 1.000 & 0.980 & 0.112 \\
image\_39.png & 1.000 & 0.980 & 0.055 \\
image\_40.png & 0.900 & 0.980 & 0.127 \\
image\_41.png & 0.970 & 0.980 & 0.048 \\
image\_42.png & 1.000 & 0.980 & 0.092 \\
image\_43.png & 1.000 & 0.980 & 0.110 \\
image\_44.png & 1.000 & 0.980 & 0.062 \\
image\_45.png & 1.000 & 0.980 & 0.129 \\
image\_46.png & 1.000 & 0.980 & 0.064 \\
image\_47.png & 0.970 & 0.990 & 0.075 \\
image\_48.png & 0.970 & 0.990 & 0.180 \\
image\_49.png & 1.000 & 0.980 & 0.069 \\
image\_50.png & 0.970 & 0.980 & 0.098 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.976 & 0.982 & 0.142 \\
\textbf{Average (CelebA, 26--50)} & 0.986 & 0.981 & 0.103 \\

\end{longtable}
\endgroup

\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lccc}
\caption{Phase 2 (StegaHiDDeN) --- Step 1: StegaStamp embedding on the benchmark dataset. Per-image bit accuracy for each decoder: $\mathrm{BA}_{\text{HiDDeN}}$ (hidden) and $\mathrm{BA}_{\text{Stega}}$ (stega), with similarity score. Images 1--25: COCO, 26--50: CelebA.}
\label{tab:phase1_stegahidden_step1_stega_embed}\\
\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & Similarity Score \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & Similarity Score \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1.png  & 0.570 & 1.000 & 0.145 \\
image\_2.png  & 0.430 & 1.000 & 0.220 \\
image\_3.png  & 0.330 & 1.000 & 0.219 \\
image\_4.png  & 0.530 & 1.000 & 0.147 \\
image\_5.png  & 0.400 & 1.000 & 0.139 \\
image\_6.png  & 0.370 & 1.000 & 0.192 \\
image\_7.png  & 0.470 & 1.000 & 0.126 \\
image\_8.png  & 0.470 & 1.000 & 0.155 \\
image\_9.png  & 0.430 & 1.000 & 0.218 \\
image\_10.png & 0.370 & 1.000 & 0.221 \\
image\_11.png & 0.400 & 1.000 & 0.148 \\
image\_12.png & 0.400 & 1.000 & 0.196 \\
image\_13.png & 0.400 & 0.990 & 0.135 \\
image\_14.png & 0.500 & 1.000 & 0.158 \\
image\_15.png & 0.430 & 1.000 & 0.191 \\
image\_16.png & 0.400 & 1.000 & 0.192 \\
image\_17.png & 0.400 & 1.000 & 0.148 \\
image\_18.png & 0.400 & 1.000 & 0.174 \\
image\_19.png & 0.430 & 1.000 & 0.170 \\
image\_20.png & 0.370 & 1.000 & 0.255 \\
image\_21.png & 0.430 & 1.000 & 0.178 \\
image\_22.png & 0.500 & 1.000 & 0.185 \\
image\_23.png & 0.430 & 0.990 & 0.192 \\
image\_24.png & 0.530 & 0.990 & 0.147 \\
image\_25.png & 0.400 & 1.000 & 0.222 \\
image\_26.png & 0.470 & 1.000 & 0.172 \\
image\_27.png & 0.400 & 1.000 & 0.186 \\
image\_28.png & 0.670 & 1.000 & 0.147 \\
image\_29.png & 0.430 & 1.000 & 0.141 \\
image\_30.png & 0.570 & 1.000 & 0.107 \\
image\_31.png & 0.430 & 1.000 & 0.125 \\
image\_32.png & 0.400 & 1.000 & 0.184 \\
image\_33.png & 0.430 & 1.000 & 0.122 \\
image\_34.png & 0.400 & 1.000 & 0.215 \\
image\_35.png & 0.470 & 1.000 & 0.125 \\
image\_36.png & 0.470 & 1.000 & 0.166 \\
image\_37.png & 0.500 & 1.000 & 0.132 \\
image\_38.png & 0.470 & 1.000 & 0.231 \\
image\_39.png & 0.500 & 1.000 & 0.104 \\
image\_40.png & 0.400 & 1.000 & 0.247 \\
image\_41.png & 0.530 & 1.000 & 0.091 \\
image\_42.png & 0.370 & 1.000 & 0.113 \\
image\_43.png & 0.500 & 1.000 & 0.134 \\
image\_44.png & 0.500 & 1.000 & 0.093 \\
image\_45.png & 0.470 & 1.000 & 0.124 \\
image\_46.png & 0.400 & 1.000 & 0.096 \\
image\_47.png & 0.500 & 1.000 & 0.086 \\
image\_48.png & 0.470 & 1.000 & 0.187 \\
image\_49.png & 0.400 & 1.000 & 0.139 \\
image\_50.png & 0.400 & 1.000 & 0.173 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.437 & 0.998 & 0.179 \\
\textbf{Average (CelebA, 26--50)} & 0.459 & 1.000 & 0.145 \\

\end{longtable}
\endgroup



\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lccc}
\caption{Phase 2 (StegaHiDDeN) --- Step 2: HiDDeN embedding on the StegaStamp-embedded dataset to create \textit{StegaHiDDeN}. Per-image bit accuracy for each decoder: $\mathrm{BA}_{\text{HiDDeN}}$ and $\mathrm{BA}_{\text{Stega}}$, with similarity score. Images 1--25: COCO, 26--50: CelebA.}
\label{tab:phase1_stegahidden_step2_hidden_embed}\\
\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & Similarity Score \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & Similarity Score \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1.png  & 1.000 & 0.980 & 0.026 \\
image\_2.png  & 1.000 & 0.990 & 0.057 \\
image\_3.png  & 1.000 & 1.000 & 0.035 \\
image\_4.png  & 1.000 & 0.980 & 0.032 \\
image\_5.png  & 1.000 & 0.990 & 0.027 \\
image\_6.png  & 1.000 & 1.000 & 0.042 \\
image\_7.png  & 1.000 & 1.000 & 0.023 \\
image\_8.png  & 1.000 & 1.000 & 0.037 \\
image\_9.png  & 1.000 & 1.000 & 0.042 \\
image\_10.png & 1.000 & 1.000 & 0.041 \\
image\_11.png & 1.000 & 0.990 & 0.031 \\
image\_12.png & 1.000 & 1.000 & 0.037 \\
image\_13.png & 1.000 & 0.990 & 0.034 \\
image\_14.png & 1.000 & 1.000 & 0.032 \\
image\_15.png & 1.000 & 0.990 & 0.031 \\
image\_16.png & 1.000 & 1.000 & 0.032 \\
image\_17.png & 1.000 & 0.970 & 0.028 \\
image\_18.png & 1.000 & 1.000 & 0.036 \\
image\_19.png & 1.000 & 1.000 & 0.042 \\
image\_20.png & 1.000 & 1.000 & 0.043 \\
image\_21.png & 1.000 & 1.000 & 0.035 \\
image\_22.png & 1.000 & 0.980 & 0.042 \\
image\_23.png & 1.000 & 0.980 & 0.040 \\
image\_24.png & 1.000 & 1.000 & 0.029 \\
image\_25.png & 1.000 & 1.000 & 0.041 \\
image\_26.png & 1.000 & 1.000 & 0.071 \\
image\_27.png & 1.000 & 0.990 & 0.065 \\
image\_28.png & 1.000 & 0.990 & 0.042 \\
image\_29.png & 1.000 & 0.980 & 0.066 \\
image\_30.png & 1.000 & 0.990 & 0.032 \\
image\_31.png & 1.000 & 1.000 & 0.041 \\
image\_32.png & 1.000 & 1.000 & 0.057 \\
image\_33.png & 1.000 & 0.980 & 0.043 \\
image\_34.png & 1.000 & 0.980 & 0.062 \\
image\_35.png & 1.000 & 0.980 & 0.056 \\
image\_36.png & 1.000 & 1.000 & 0.058 \\
image\_37.png & 1.000 & 0.980 & 0.036 \\
image\_38.png & 1.000 & 1.000 & 0.051 \\
image\_39.png & 0.970 & 1.000 & 0.032 \\
image\_40.png & 1.000 & 1.000 & 0.092 \\
image\_41.png & 0.970 & 1.000 & 0.026 \\
image\_42.png & 1.000 & 1.000 & 0.035 \\
image\_43.png & 1.000 & 0.990 & 0.037 \\
image\_44.png & 1.000 & 0.990 & 0.025 \\
image\_45.png & 1.000 & 1.000 & 0.038 \\
image\_46.png & 1.000 & 0.980 & 0.028 \\
image\_47.png & 0.970 & 0.980 & 0.026 \\
image\_48.png & 1.000 & 1.000 & 0.076 \\
image\_49.png & 0.970 & 1.000 & 0.059 \\
image\_50.png & 1.000 & 1.000 & 0.051 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 1.000 & 0.994 & 0.035 \\
\textbf{Average (CelebA, 26--50)} & 0.993 & 0.992 & 0.052 \\

\end{longtable}


\endgroup

\subsection{Phase 3: Dual attack sequence study}
\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lccc}
\caption{Non-semantic attack on \textit{HiDDeNStega} dataset. Per-image bit accuracy for each decoder: $\mathrm{BA}_{\text{HiDDeN}}$ and $\mathrm{BA}_{\text{Stega}}$, with LPIPS (Similarity Score). Images 1--25: COCO, 26--50: CelebA.}
\label{tab:P3_HS_NS}\\
\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1.png  & 0.600 & 0.940 & 0.007 \\
image\_2.png  & 0.600 & 0.960 & 0.012 \\
image\_3.png  & 0.530 & 0.940 & 0.008 \\
image\_4.png  & 0.770 & 0.930 & 0.008 \\
image\_5.png  & 0.530 & 0.980 & 0.006 \\
image\_6.png  & 0.600 & 0.970 & 0.008 \\
image\_7.png  & 0.630 & 0.970 & 0.007 \\
image\_8.png  & 0.630 & 0.960 & 0.009 \\
image\_9.png  & 0.600 & 0.920 & 0.010 \\
image\_10.png & 0.670 & 0.960 & 0.010 \\
image\_11.png & 0.570 & 0.960 & 0.009 \\
image\_12.png & 0.600 & 0.960 & 0.010 \\
image\_13.png & 0.570 & 0.970 & 0.008 \\
image\_14.png & 0.530 & 0.980 & 0.008 \\
image\_15.png & 0.470 & 0.980 & 0.008 \\
image\_16.png & 0.600 & 0.940 & 0.008 \\
image\_17.png & 0.500 & 0.960 & 0.007 \\
image\_18.png & 0.600 & 0.950 & 0.009 \\
image\_19.png & 0.600 & 0.950 & 0.011 \\
image\_20.png & 0.570 & 0.950 & 0.009 \\
image\_21.png & 0.630 & 0.970 & 0.008 \\
image\_22.png & 0.570 & 0.970 & 0.008 \\
image\_23.png & 0.500 & 0.850 & 0.008 \\
image\_24.png & 0.570 & 0.950 & 0.008 \\
image\_25.png & 0.570 & 0.980 & 0.008 \\
image\_26.png & 0.530 & 0.970 & 0.014 \\
image\_27.png & 0.630 & 0.890 & 0.010 \\
image\_28.png & 0.530 & 0.970 & 0.009 \\
image\_29.png & 0.770 & 0.990 & 0.008 \\
image\_30.png & 0.500 & 0.970 & 0.008 \\
image\_31.png & 0.570 & 0.950 & 0.012 \\
image\_32.png & 0.700 & 0.910 & 0.011 \\
image\_33.png & 0.570 & 0.980 & 0.011 \\
image\_34.png & 0.600 & 0.970 & 0.009 \\
image\_35.png & 0.700 & 0.990 & 0.011 \\
image\_36.png & 0.730 & 0.900 & 0.008 \\
image\_37.png & 0.500 & 0.970 & 0.013 \\
image\_38.png & 0.530 & 0.950 & 0.011 \\
image\_39.png & 0.600 & 0.960 & 0.005 \\
image\_40.png & 0.530 & 0.970 & 0.011 \\
image\_41.png & 0.670 & 0.950 & 0.007 \\
image\_42.png & 0.630 & 0.970 & 0.011 \\
image\_43.png & 0.570 & 0.980 & 0.010 \\
image\_44.png & 0.670 & 0.970 & 0.011 \\
image\_45.png & 0.730 & 0.970 & 0.007 \\
image\_46.png & 0.600 & 0.960 & 0.011 \\
image\_47.png & 0.730 & 0.960 & 0.008 \\
image\_48.png & 0.570 & 1.000 & 0.016 \\
image\_49.png & 0.630 & 0.970 & 0.007 \\
image\_50.png & 0.570 & 0.930 & 0.012 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.584 & 0.954 & 0.009 \\
\textbf{Average (CelebA, 26--50)} & 0.614 & 0.960 & 0.010 \\
\textbf{Average (Overall, 1--50)} & 0.599 & 0.957 & 0.009 \\

\end{longtable}
\endgroup


\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lccc}
\caption{Semantic attack on the \textit{HiDDeNStega} dataset \textbf{after} a non-semantic attack (i.e., Non-semantic $\rightarrow$ semantic). Per-image bit accuracy for each decoder: $\mathrm{BA}_{\text{HiDDeN}}$ and $\mathrm{BA}_{\text{Stega}}$, with LPIPS (Similarity Score). Images 1--25: COCO, 26--50: CelebA.}
\label{tab:p3_HS_NS_S}\\
\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1.png  & 0.630 & 0.640 & 0.071 \\
image\_2.png  & 0.600 & 0.650 & 0.111 \\
image\_3.png  & 0.430 & 0.690 & 0.067 \\
image\_4.png  & 0.700 & 0.820 & 0.068 \\
image\_5.png  & 0.530 & 0.750 & 0.055 \\
image\_6.png  & 0.530 & 0.740 & 0.086 \\
image\_7.png  & 0.600 & 0.770 & 0.068 \\
image\_8.png  & 0.630 & 0.790 & 0.065 \\
image\_9.png  & 0.570 & 0.670 & 0.096 \\
image\_10.png & 0.600 & 0.800 & 0.098 \\
image\_11.png & 0.530 & 0.750 & 0.071 \\
image\_12.png & 0.570 & 0.710 & 0.084 \\
image\_13.png & 0.500 & 0.640 & 0.066 \\
image\_14.png & 0.530 & 0.810 & 0.069 \\
image\_15.png & 0.470 & 0.690 & 0.086 \\
image\_16.png & 0.570 & 0.770 & 0.078 \\
image\_17.png & 0.430 & 0.680 & 0.087 \\
image\_18.png & 0.500 & 0.650 & 0.088 \\
image\_19.png & 0.530 & 0.630 & 0.100 \\
image\_20.png & 0.530 & 0.780 & 0.090 \\
image\_21.png & 0.600 & 0.760 & 0.083 \\
image\_22.png & 0.570 & 0.790 & 0.087 \\
image\_23.png & 0.530 & 0.710 & 0.083 \\
image\_24.png & 0.600 & 0.620 & 0.078 \\
image\_25.png & 0.570 & 0.690 & 0.101 \\
image\_26.png & 0.530 & 0.480 & 0.112 \\
image\_27.png & 0.600 & 0.530 & 0.105 \\
image\_28.png & 0.530 & 0.720 & 0.065 \\
image\_29.png & 0.670 & 0.680 & 0.083 \\
image\_30.png & 0.530 & 0.700 & 0.064 \\
image\_31.png & 0.600 & 0.580 & 0.097 \\
image\_32.png & 0.630 & 0.600 & 0.089 \\
image\_33.png & 0.570 & 0.640 & 0.091 \\
image\_34.png & 0.630 & 0.890 & 0.116 \\
image\_35.png & 0.630 & 0.560 & 0.103 \\
image\_36.png & 0.700 & 0.660 & 0.076 \\
image\_37.png & 0.470 & 0.710 & 0.092 \\
image\_38.png & 0.530 & 0.640 & 0.102 \\
image\_39.png & 0.600 & 0.930 & 0.033 \\
image\_40.png & 0.470 & 0.660 & 0.122 \\
image\_41.png & 0.670 & 0.650 & 0.048 \\
image\_42.png & 0.600 & 0.640 & 0.084 \\
image\_43.png & 0.570 & 0.580 & 0.085 \\
image\_44.png & 0.600 & 0.740 & 0.065 \\
image\_45.png & 0.730 & 0.670 & 0.062 \\
image\_46.png & 0.600 & 0.600 & 0.073 \\
image\_47.png & 0.670 & 0.790 & 0.061 \\
image\_48.png & 0.530 & 0.670 & 0.139 \\
image\_49.png & 0.630 & 0.610 & 0.080 \\
image\_50.png & 0.530 & 0.500 & 0.081 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.554 & 0.720 & 0.081 \\
\textbf{Average (CelebA, 26--50)} & 0.593 & 0.657 & 0.085 \\
\textbf{Average (Overall, 1--50)} & 0.573 & 0.689 & 0.083 \\

\end{longtable}
\endgroup


\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lccc}
\caption{Semantic attack on \textit{HiDDeNStega} dataset. Per-image bit accuracy for each decoder: $\mathrm{BA}_{\text{HiDDeN}}$ and $\mathrm{BA}_{\text{Stega}}$, with LPIPS (Similarity Score). Images 1--25: COCO, 26--50: CelebA.}
\label{tab:P3_HS_S}\\
\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1.png  & 0.900 & 0.610 & 0.075 \\
image\_2.png  & 0.670 & 0.630 & 0.116 \\
image\_3.png  & 0.830 & 0.640 & 0.076 \\
image\_4.png  & 1.000 & 0.730 & 0.075 \\
image\_5.png  & 0.900 & 0.790 & 0.061 \\
image\_6.png  & 0.900 & 0.700 & 0.090 \\
image\_7.png  & 0.930 & 0.760 & 0.072 \\
image\_8.png  & 0.870 & 0.730 & 0.068 \\
image\_9.png  & 0.870 & 0.580 & 0.106 \\
image\_10.png & 0.870 & 0.750 & 0.101 \\
image\_11.png & 0.900 & 0.680 & 0.079 \\
image\_12.png & 0.830 & 0.610 & 0.094 \\
image\_13.png & 0.800 & 0.640 & 0.076 \\
image\_14.png & 0.870 & 0.700 & 0.079 \\
image\_15.png & 0.700 & 0.730 & 0.087 \\
image\_16.png & 0.900 & 0.690 & 0.084 \\
image\_17.png & 0.800 & 0.660 & 0.092 \\
image\_18.png & 0.870 & 0.620 & 0.094 \\
image\_19.png & 0.900 & 0.630 & 0.102 \\
image\_20.png & 0.830 & 0.700 & 0.097 \\
image\_21.png & 0.870 & 0.700 & 0.087 \\
image\_22.png & 0.900 & 0.680 & 0.092 \\
image\_23.png & 0.770 & 0.640 & 0.090 \\
image\_24.png & 0.930 & 0.590 & 0.086 \\
image\_25.png & 0.830 & 0.580 & 0.102 \\
image\_26.png & 0.930 & 0.580 & 0.094 \\
image\_27.png & 0.930 & 0.580 & 0.079 \\
image\_28.png & 0.870 & 0.560 & 0.064 \\
image\_29.png & 0.970 & 0.620 & 0.087 \\
image\_30.png & 0.930 & 0.580 & 0.065 \\
image\_31.png & 0.970 & 0.550 & 0.076 \\
image\_32.png & 0.900 & 0.580 & 0.066 \\
image\_33.png & 0.870 & 0.610 & 0.097 \\
image\_34.png & 0.830 & 0.880 & 0.120 \\
image\_35.png & 0.930 & 0.580 & 0.082 \\
image\_36.png & 0.900 & 0.630 & 0.083 \\
image\_37.png & 0.970 & 0.580 & 0.083 \\
image\_38.png & 0.900 & 0.650 & 0.112 \\
image\_39.png & 0.930 & 0.810 & 0.041 \\
image\_40.png & 0.730 & 0.570 & 0.109 \\
image\_41.png & 0.970 & 0.650 & 0.058 \\
image\_42.png & 0.930 & 0.570 & 0.072 \\
image\_43.png & 1.000 & 0.580 & 0.064 \\
image\_44.png & 0.930 & 0.610 & 0.073 \\
image\_45.png & 0.930 & 0.570 & 0.055 \\
image\_46.png & 0.970 & 0.580 & 0.066 \\
image\_47.png & 0.900 & 0.680 & 0.071 \\
image\_48.png & 0.700 & 0.580 & 0.123 \\
image\_49.png & 0.870 & 0.580 & 0.073 \\
image\_50.png & 0.970 & 0.570 & 0.078 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.858 & 0.671 & 0.087 \\
\textbf{Average (CelebA, 26--50)} & 0.909 & 0.613 & 0.080 \\
\textbf{Average (Overall, 1--50)} & 0.883 & 0.642 & 0.083 \\

\end{longtable}
\endgroup


\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lccc}
\caption{Non-semantic attack on the \textit{HiDDeNStega} dataset \textbf{after} a semantic attack (i.e., Semantic $\rightarrow$ Non-semantic). Per-image bit accuracy for each decoder: $\mathrm{BA}_{\text{HiDDeN}}$ and $\mathrm{BA}_{\text{Stega}}$, with LPIPS (Similarity Score). Images 1--25: COCO, 26--50: CelebA.}
\label{tab:P3_HS_S_NS}\\
\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1.png  & 0.630 & 0.660 & 0.007 \\
image\_2.png  & 0.570 & 0.650 & 0.008 \\
image\_3.png  & 0.570 & 0.680 & 0.006 \\
image\_4.png  & 0.730 & 0.740 & 0.008 \\
image\_5.png  & 0.600 & 0.760 & 0.006 \\
image\_6.png  & 0.570 & 0.730 & 0.006 \\
image\_7.png  & 0.600 & 0.730 & 0.007 \\
image\_8.png  & 0.670 & 0.690 & 0.009 \\
image\_9.png  & 0.570 & 0.590 & 0.007 \\
image\_10.png & 0.570 & 0.780 & 0.006 \\
image\_11.png & 0.570 & 0.730 & 0.007 \\
image\_12.png & 0.570 & 0.620 & 0.007 \\
image\_13.png & 0.570 & 0.630 & 0.006 \\
image\_14.png & 0.570 & 0.770 & 0.006 \\
image\_15.png & 0.570 & 0.700 & 0.005 \\
image\_16.png & 0.600 & 0.700 & 0.008 \\
image\_17.png & 0.570 & 0.620 & 0.003 \\
image\_18.png & 0.570 & 0.600 & 0.006 \\
image\_19.png & 0.630 & 0.600 & 0.010 \\
image\_20.png & 0.570 & 0.750 & 0.007 \\
image\_21.png & 0.530 & 0.720 & 0.007 \\
image\_22.png & 0.630 & 0.740 & 0.008 \\
image\_23.png & 0.600 & 0.720 & 0.008 \\
image\_24.png & 0.570 & 0.540 & 0.007 \\
image\_25.png & 0.570 & 0.630 & 0.006 \\
image\_26.png & 0.570 & 0.600 & 0.012 \\
image\_27.png & 0.600 & 0.590 & 0.010 \\
image\_28.png & 0.570 & 0.610 & 0.006 \\
image\_29.png & 0.670 & 0.630 & 0.007 \\
image\_30.png & 0.570 & 0.580 & 0.008 \\
image\_31.png & 0.630 & 0.610 & 0.013 \\
image\_32.png & 0.700 & 0.670 & 0.011 \\
image\_33.png & 0.570 & 0.590 & 0.007 \\
image\_34.png & 0.570 & 0.870 & 0.009 \\
image\_35.png & 0.630 & 0.610 & 0.012 \\
image\_36.png & 0.670 & 0.720 & 0.007 \\
image\_37.png & 0.570 & 0.610 & 0.008 \\
image\_38.png & 0.570 & 0.630 & 0.008 \\
image\_39.png & 0.670 & 0.850 & 0.005 \\
image\_40.png & 0.570 & 0.640 & 0.005 \\
image\_41.png & 0.700 & 0.670 & 0.007 \\
image\_42.png & 0.630 & 0.580 & 0.011 \\
image\_43.png & 0.630 & 0.610 & 0.011 \\
image\_44.png & 0.700 & 0.600 & 0.011 \\
image\_45.png & 0.700 & 0.610 & 0.007 \\
image\_46.png & 0.630 & 0.620 & 0.011 \\
image\_47.png & 0.670 & 0.710 & 0.008 \\
image\_48.png & 0.570 & 0.640 & 0.009 \\
image\_49.png & 0.630 & 0.590 & 0.008 \\
image\_50.png & 0.570 & 0.560 & 0.008 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.591 & 0.683 & 0.007 \\
\textbf{Average (CelebA, 26--50)} & 0.622 & 0.640 & 0.009 \\
\textbf{Average (Overall, 1--50)} & 0.607 & 0.662 & 0.008 \\

\end{longtable}
\endgroup


\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lccc}
\caption{Non-semantic attack on the \textit{StegaHiDDeN} dataset. Per-image bit accuracy for each decoder: $\mathrm{BA}_{\text{HiDDeN}}$ and $\mathrm{BA}_{\text{Stega}}$, with LPIPS (Similarity Score). Images 1--25: COCO, 26--50: CelebA.}
\label{tab:P3_SH_NS}\\
\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1.png  & 0.570 & 1.000 & 0.007 \\
image\_2.png  & 0.670 & 0.990 & 0.016 \\
image\_3.png  & 0.600 & 1.000 & 0.008 \\
image\_4.png  & 0.730 & 0.950 & 0.008 \\
image\_5.png  & 0.670 & 0.970 & 0.006 \\
image\_6.png  & 0.600 & 1.000 & 0.007 \\
image\_7.png  & 0.600 & 1.000 & 0.007 \\
image\_8.png  & 0.700 & 1.000 & 0.010 \\
image\_9.png  & 0.670 & 1.000 & 0.012 \\
image\_10.png & 0.700 & 1.000 & 0.009 \\
image\_11.png & 0.600 & 0.990 & 0.010 \\
image\_12.png & 0.570 & 1.000 & 0.009 \\
image\_13.png & 0.670 & 0.980 & 0.008 \\
image\_14.png & 0.600 & 1.000 & 0.008 \\
image\_15.png & 0.670 & 0.990 & 0.011 \\
image\_16.png & 0.670 & 1.000 & 0.008 \\
image\_17.png & 0.630 & 0.950 & 0.009 \\
image\_18.png & 0.600 & 0.990 & 0.009 \\
image\_19.png & 0.700 & 0.990 & 0.013 \\
image\_20.png & 0.700 & 1.000 & 0.011 \\
image\_21.png & 0.670 & 1.000 & 0.008 \\
image\_22.png & 0.570 & 0.990 & 0.008 \\
image\_23.png & 0.700 & 0.930 & 0.008 \\
image\_24.png & 0.570 & 1.000 & 0.008 \\
image\_25.png & 0.570 & 1.000 & 0.009 \\
image\_26.png & 0.570 & 1.000 & 0.011 \\
image\_27.png & 0.630 & 0.980 & 0.010 \\
image\_28.png & 0.530 & 0.990 & 0.007 \\
image\_29.png & 0.830 & 0.970 & 0.008 \\
image\_30.png & 0.630 & 0.980 & 0.009 \\
image\_31.png & 0.700 & 0.990 & 0.012 \\
image\_32.png & 0.730 & 1.000 & 0.011 \\
image\_33.png & 0.600 & 0.980 & 0.010 \\
image\_34.png & 0.670 & 0.990 & 0.008 \\
image\_35.png & 0.730 & 0.990 & 0.011 \\
image\_36.png & 0.730 & 0.990 & 0.007 \\
image\_37.png & 0.670 & 0.950 & 0.014 \\
image\_38.png & 0.570 & 1.000 & 0.011 \\
image\_39.png & 0.670 & 1.000 & 0.006 \\
image\_40.png & 0.670 & 1.000 & 0.011 \\
image\_41.png & 0.730 & 1.000 & 0.006 \\
image\_42.png & 0.700 & 0.990 & 0.010 \\
image\_43.png & 0.630 & 0.990 & 0.010 \\
image\_44.png & 0.770 & 0.980 & 0.010 \\
image\_45.png & 0.770 & 1.000 & 0.007 \\
image\_46.png & 0.670 & 0.990 & 0.010 \\
image\_47.png & 0.730 & 0.950 & 0.008 \\
image\_48.png & 0.700 & 1.000 & 0.017 \\
image\_49.png & 0.730 & 1.000 & 0.006 \\
image\_50.png & 0.570 & 0.980 & 0.011 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.640 & 0.989 & 0.009 \\
\textbf{Average (CelebA, 26--50)} & 0.677 & 0.988 & 0.010 \\
\textbf{Average (Overall, 1--50)} & 0.659 & 0.988 & 0.009 \\

\end{longtable}
\endgroup



\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lccc}
\caption{Semantic attack on the \textit{StegaHiDDeN} dataset \textbf{after} a non-semantic attack (i.e., Non-semantic $\rightarrow$ Semantic). Per-image bit accuracy for each decoder: $\mathrm{BA}_{\text{HiDDeN}}$ and $\mathrm{BA}_{\text{Stega}}$, with LPIPS (Similarity Score). Images 1--25: COCO, 26--50: CelebA.}
\label{tab:P3_SH_NS_S}\\
\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1.png  & 0.600 & 0.570 & 0.151 \\
image\_2.png  & 0.600 & 0.630 & 0.198 \\
image\_3.png  & 0.600 & 0.620 & 0.132 \\
image\_4.png  & 0.670 & 0.630 & 0.155 \\
image\_5.png  & 0.670 & 0.610 & 0.119 \\
image\_6.png  & 0.570 & 0.610 & 0.171 \\
image\_7.png  & 0.570 & 0.620 & 0.150 \\
image\_8.png  & 0.630 & 0.670 & 0.160 \\
image\_9.png  & 0.630 & 0.630 & 0.205 \\
image\_10.png & 0.630 & 0.580 & 0.168 \\
image\_11.png & 0.530 & 0.680 & 0.142 \\
image\_12.png & 0.530 & 0.630 & 0.155 \\
image\_13.png & 0.570 & 0.660 & 0.144 \\
image\_14.png & 0.630 & 0.690 & 0.131 \\
image\_15.png & 0.670 & 0.640 & 0.181 \\
image\_16.png & 0.670 & 0.710 & 0.171 \\
image\_17.png & 0.630 & 0.580 & 0.123 \\
image\_18.png & 0.500 & 0.560 & 0.134 \\
image\_19.png & 0.630 & 0.570 & 0.166 \\
image\_20.png & 0.630 & 0.580 & 0.195 \\
image\_21.png & 0.570 & 0.700 & 0.175 \\
image\_22.png & 0.570 & 0.570 & 0.131 \\
image\_23.png & 0.570 & 0.580 & 0.153 \\
image\_24.png & 0.630 & 0.580 & 0.120 \\
image\_25.png & 0.570 & 0.580 & 0.149 \\
image\_26.png & 0.570 & 0.580 & 0.175 \\
image\_27.png & 0.570 & 0.570 & 0.129 \\
image\_28.png & 0.600 & 0.580 & 0.110 \\
image\_29.png & 0.800 & 0.580 & 0.130 \\
image\_30.png & 0.630 & 0.690 & 0.144 \\
image\_31.png & 0.600 & 0.550 & 0.115 \\
image\_32.png & 0.730 & 0.570 & 0.116 \\
image\_33.png & 0.600 & 0.580 & 0.134 \\
image\_34.png & 0.470 & 0.650 & 0.195 \\
image\_35.png & 0.630 & 0.570 & 0.113 \\
image\_36.png & 0.670 & 0.580 & 0.114 \\
image\_37.png & 0.630 & 0.650 & 0.187 \\
image\_38.png & 0.530 & 0.660 & 0.167 \\
image\_39.png & 0.630 & 0.860 & 0.090 \\
image\_40.png & 0.570 & 0.530 & 0.161 \\
image\_41.png & 0.770 & 0.700 & 0.108 \\
image\_42.png & 0.530 & 0.590 & 0.176 \\
image\_43.png & 0.670 & 0.650 & 0.159 \\
image\_44.png & 0.630 & 0.720 & 0.168 \\
image\_45.png & 0.700 & 0.570 & 0.106 \\
image\_46.png & 0.670 & 0.580 & 0.101 \\
image\_47.png & 0.730 & 0.620 & 0.133 \\
image\_48.png & 0.630 & 0.570 & 0.200 \\
image\_49.png & 0.570 & 0.610 & 0.141 \\
image\_50.png & 0.570 & 0.550 & 0.124 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.603 & 0.619 & 0.155 \\
\textbf{Average (CelebA, 26--50)} & 0.628 & 0.614 & 0.140 \\
\textbf{Average (Overall, 1--50)} & 0.615 & 0.617 & 0.148 \\

\end{longtable}
\endgroup

\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lccc}
\caption{Semantic attack on the \textit{StegaHiDDeN} dataset. Per-image bit accuracy for each decoder: $\mathrm{BA}_{\text{HiDDeN}}$ and $\mathrm{BA}_{\text{Stega}}$, with LPIPS (Similarity Score). Images 1--25: COCO, 26--50: CelebA.}
\label{tab:P3_SH_S}\\
\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1.png & 0.900 & 0.580 & 0.127 \\
image\_2.png & 0.830 & 0.580 & 0.199 \\
image\_3.png & 0.900 & 0.580 & 0.100 \\
image\_4.png & 0.830 & 0.570 & 0.162 \\
image\_5.png & 0.900 & 0.580 & 0.117 \\
image\_6.png & 0.930 & 0.570 & 0.131 \\
image\_7.png & 0.830 & 0.570 & 0.141 \\
image\_8.png & 0.770 & 0.660 & 0.180 \\
image\_9.png & 0.930 & 0.570 & 0.145 \\
image\_10.png & 0.730 & 0.600 & 0.214 \\
image\_11.png & 0.900 & 0.580 & 0.123 \\
image\_12.png & 0.930 & 0.580 & 0.124 \\
image\_13.png & 0.930 & 0.580 & 0.132 \\
image\_14.png & 0.830 & 0.580 & 0.128 \\
image\_15.png & 0.730 & 0.600 & 0.183 \\
image\_16.png & 0.930 & 0.580 & 0.120 \\
image\_17.png & 1.000 & 0.580 & 0.118 \\
image\_18.png & 0.970 & 0.550 & 0.119 \\
image\_19.png & 0.900 & 0.570 & 0.157 \\
image\_20.png & 0.800 & 0.580 & 0.191 \\
image\_21.png & 0.830 & 0.580 & 0.136 \\
image\_22.png & 0.970 & 0.580 & 0.147 \\
image\_23.png & 0.870 & 0.570 & 0.167 \\
image\_24.png & 0.930 & 0.580 & 0.119 \\
image\_25.png & 0.930 & 0.580 & 0.130 \\
image\_26.png & 0.930 & 0.580 & 0.146 \\
image\_27.png & 0.930 & 0.580 & 0.125 \\
image\_28.png & 0.870 & 0.580 & 0.099 \\
image\_29.png & 0.970 & 0.580 & 0.141 \\
image\_30.png & 0.930 & 0.570 & 0.102 \\
image\_31.png & 0.970 & 0.540 & 0.116 \\
image\_32.png & 0.900 & 0.580 & 0.137 \\
image\_33.png & 0.970 & 0.580 & 0.143 \\
image\_34.png & 0.730 & 0.700 & 0.242 \\
image\_35.png & 0.930 & 0.570 & 0.135 \\
image\_36.png & 0.970 & 0.580 & 0.127 \\
image\_37.png & 1.000 & 0.560 & 0.122 \\
image\_38.png & 0.730 & 0.570 & 0.170 \\
image\_39.png & 0.800 & 0.620 & 0.112 \\
image\_40.png & 0.830 & 0.580 & 0.150 \\
image\_41.png & 0.970 & 0.580 & 0.080 \\
image\_42.png & 0.930 & 0.550 & 0.124 \\
image\_43.png & 0.970 & 0.560 & 0.089 \\
image\_44.png & 0.930 & 0.580 & 0.104 \\
image\_45.png & 0.930 & 0.580 & 0.086 \\
image\_46.png & 0.970 & 0.580 & 0.114 \\
image\_47.png & 0.930 & 0.570 & 0.115 \\
image\_48.png & 0.870 & 0.570 & 0.195 \\
image\_49.png & 0.930 & 0.580 & 0.104 \\
image\_50.png & 0.970 & 0.580 & 0.110 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.880 & 0.581 & 0.144 \\
\textbf{Average (CelebA, 26--50)} & 0.914 & 0.580 & 0.128 \\
\textbf{Average (Overall, 1--50)} & 0.897 & 0.581 & 0.136 \\

\end{longtable}
\endgroup


\begingroup
\small
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{0.95}

\begin{longtable}{lccc}
\caption{Non-semantic attack on the \textit{StegaHiDDeN} dataset \textbf{after} a Semantic attack (i.e., Semantic $\rightarrow$ Non-semantic). Per-image bit accuracy for each decoder: $\mathrm{BA}_{\text{HiDDeN}}$ and $\mathrm{BA}_{\text{Stega}}$, with LPIPS (Similarity Score). Images 1--25: COCO, 26--50: CelebA.}
\label{tab:P3_SH_S_NS}\\
\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endfirsthead

\toprule
Image & $\mathrm{BA}_{\text{HiDDeN}}$ & $\mathrm{BA}_{\text{Stega}}$ & LPIPS \\
\midrule
\endhead

\midrule
\multicolumn{4}{r}{\textit{Continued on next page}}\\
\endfoot

\bottomrule
\endlastfoot

image\_1.png  & 0.570 & 0.550 & 0.007 \\
image\_2.png  & 0.630 & 0.590 & 0.011 \\
image\_3.png  & 0.570 & 0.540 & 0.008 \\
image\_4.png  & 0.670 & 0.580 & 0.007 \\
image\_5.png  & 0.670 & 0.610 & 0.006 \\
image\_6.png  & 0.570 & 0.550 & 0.008 \\
image\_7.png  & 0.670 & 0.610 & 0.007 \\
image\_8.png  & 0.630 & 0.720 & 0.008 \\
image\_9.png  & 0.600 & 0.560 & 0.011 \\
image\_10.png & 0.600 & 0.600 & 0.008 \\
image\_11.png & 0.600 & 0.620 & 0.009 \\
image\_12.png & 0.600 & 0.650 & 0.009 \\
image\_13.png & 0.570 & 0.610 & 0.009 \\
image\_14.png & 0.570 & 0.620 & 0.007 \\
image\_15.png & 0.630 & 0.590 & 0.009 \\
image\_16.png & 0.570 & 0.540 & 0.008 \\
image\_17.png & 0.600 & 0.530 & 0.011 \\
image\_18.png & 0.530 & 0.590 & 0.009 \\
image\_19.png & 0.630 & 0.570 & 0.013 \\
image\_20.png & 0.570 & 0.590 & 0.008 \\
image\_21.png & 0.530 & 0.580 & 0.009 \\
image\_22.png & 0.630 & 0.640 & 0.008 \\
image\_23.png & 0.600 & 0.580 & 0.007 \\
image\_24.png & 0.630 & 0.610 & 0.009 \\
image\_25.png & 0.600 & 0.610 & 0.010 \\
image\_26.png & 0.600 & 0.530 & 0.013 \\
image\_27.png & 0.530 & 0.600 & 0.010 \\
image\_28.png & 0.570 & 0.590 & 0.008 \\
image\_29.png & 0.800 & 0.620 & 0.008 \\
image\_30.png & 0.630 & 0.560 & 0.009 \\
image\_31.png & 0.570 & 0.580 & 0.015 \\
image\_32.png & 0.500 & 0.600 & 0.010 \\
image\_33.png & 0.630 & 0.550 & 0.011 \\
image\_34.png & 0.530 & 0.670 & 0.008 \\
image\_35.png & 0.700 & 0.590 & 0.012 \\
image\_36.png & 0.670 & 0.580 & 0.007 \\
image\_37.png & 0.570 & 0.610 & 0.014 \\
image\_38.png & 0.500 & 0.560 & 0.008 \\
image\_39.png & 0.630 & 0.630 & 0.005 \\
image\_40.png & 0.570 & 0.630 & 0.012 \\
image\_41.png & 0.770 & 0.600 & 0.007 \\
image\_42.png & 0.630 & 0.550 & 0.012 \\
image\_43.png & 0.700 & 0.600 & 0.010 \\
image\_44.png & 0.700 & 0.560 & 0.011 \\
image\_45.png & 0.730 & 0.620 & 0.007 \\
image\_46.png & 0.670 & 0.630 & 0.011 \\
image\_47.png & 0.630 & 0.630 & 0.009 \\
image\_48.png & 0.600 & 0.610 & 0.017 \\
image\_49.png & 0.570 & 0.620 & 0.007 \\
image\_50.png & 0.530 & 0.560 & 0.013 \\

\midrule
\textbf{Average (COCO, 1--25)}     & 0.602 & 0.594 & 0.009 \\
\textbf{Average (CelebA, 26--50)} & 0.621 & 0.595 & 0.010 \\
\textbf{Average (Overall, 1--50)} & 0.611 & 0.594 & 0.009 \\

\end{longtable}
\endgroup

==> sections/02_technical_foundations.tex <==
\section{Technical foundations} \label{chap:technical-foundations}
This chapter provides the mathematical and theoretical aspects of how watermarking schemes have developed in recent years. Furthermore, it also emphasises how the UnMarker successfully attacks these watermarks (WM). In this section, the reader goes step by step to understand the complex mathematical dynamics of how watermarking schemes work, thereby also enabling the reader to understand later on how UnMarker targets the digital signatures embedded by these WMs and eventually remove them. Firstly, the mathematical basics to understand these WMs are explained. Then, the WMs are explained in details one by one. Lastly, a description of how the UnMarker targets these digital signatures are presented.


\subsection{{Mathematical basics}}
Watermarking schemes are heavily mathematical. Hence, before exploring how each WM works, the reader needs to understand the basic mathematical formulations that underlie the creation of these complex watermarking schemes.

The basics can be broken down into four steps: Images as Tensors, Loss Functions, Fourier Transforms, Convolution, and Constrained Optimization

\subsubsection{Images as tensors}
Consider an image of height, H, and width, W. In mathematical terms, this image can be represented as I is HXW. Considering grayscale images, they only have 1 channel, and thus, it is not important. However, colored images, formally known as RGB images have 3 channels, i.e., red, green, and blue. Thus, images in mathematics are formally represented as shown in Equation \ref{eq:image_tensor_representation}.

\begin{equation}
    I \in \mathbb{R}^{H \times W \times C},
    \qquad 
    C = 
    \begin{cases}
        1, & \text{grayscale},\\[4pt]
        3, & \text{RGB}.
    \end{cases}
    \label{eq:image_tensor_representation}
\end{equation}



Neural Networks treat images as tensors (vectors). Frequency Transforms (FT) treat images as functions from a 2D grid of numbers, also called pixels. Therefore, an RGB image I(x, y) can be shown as displayed in Equation \ref{eq:image_function_representation}.

\begin{equation}
\resizebox{0.90\columnwidth}{!}{$\displaystyle
    I(x, y) = 
    \begin{bmatrix}
        I_{R}(x, y) \\
        I_{G}(x, y) \\
        I_{B}(x, y)
    \end{bmatrix},
    \qquad 
    (x, y) \in \{1,\dots,H\} \times \{1,\dots,W\}.
$}
    \label{eq:image_function_representation}
\end{equation}


Watermarks modify the numerical entries in these grids or pixels. Humans can only detect structures like edges, patterns, and shapes. Thus, small modifications in pixel values are crucial for hiding watermarks beyond the human visible range. Watermarks are typically hidden in these unused tensors at frequencies that are not in the visible range of humans.

\subsubsection{Loss functions}
Loss Functions provide constraints; UnMarker uses these constraints to attack the watermarks. Each loss function has a probabilistic derivation. Therefore, these probabilistic derivations enforce a constraint on the loss function, thus creating a \textbf{predictable weakness}. UnMarker attacks target these weaknesses to remove the digital signatures embedded by WMs.


Generally, three loss functions are the most important for WM schemes. They are Mean Squared Error Loss, Cross Entropy/ Bit Reconstruction Loss and Perceptual Loss / Learned Perceptual Image Patch Similarity (LPIPS).


\paragraph{Mean squared error}
The mean square error for the watermarking scheme refers to the difference in pixel values between the original image, I, and the watermarked image, $I_{WM}$. The equation can be represented as shown in Equation \ref{eq:mse_watermarking}. 

\begin{equation}
    \text{MSE}(I, I_{\text{WM}}) 
    = \frac{1}{H\,W} 
      \sum_{x=1}^{H} \sum_{y=1}^{W} 
      \left( I(x,y) - I_{\text{WM}}(x,y) \right)^{2}
    \label{eq:mse_watermarking}
\end{equation}

From the above equation, it can be understood that if pixel values are similar the MSE is small and vice versa. This is what creates the constraint in the MSE. Watermarks add tiny noise (Gaussian Noise) to image. These noises typically minimize the MSE while adding these watermarks. Thus, the changes in MSE are small for all watermarking schemes. These changes also need to be invisible to the human eye. Therefore, the two constrains (minimal MSE and invisibility) means that the changes must be made at a minimal level in frequency ranges above the visual spectrum (high frequency). Hence, MSE for watermarking schemes only enable high frequency areas to be manipulated by watermarkers. 

This is an extremely important finding for UnMarker. UnMarker attacks these frequencies aggressively to distort the $I_{WM}$ in such a way that the decoder fails to identify the watermarks. Since, the frequency is high, after the UnMarker attack, the change in MSE is also minimal after WM removal. Additionally, for the same mentioned reason there is also no visual change on the image as these frequencies are beyond the visual spectrum. This constrain makes it easy for the UnMarker to attack MSE loss-based watermarks.

\paragraph{Cross entropy loss}
In watermarking, Encoder adds a watermark to images. Decoder then reads the watermark to provide results regarding if an image is created by AI or not. 

Encoders provides digital signatures as a sequence of binary digits. However, the decoder can only output probabilities of the digits. In order to minimize the cross-entropy (CE) loss, the decoder probabilities must correctly identify and provide probabilities close to 0 or 1. If not, the cross-entropy loss will explode. To make sure the loss does not explode, the WM Encoder must create digital patterns which are \textbf{stable and consistent patterns.} 

During distortions, i.e., compression, resizing, and noise addition, frequency components are not affected uniformly. Some parts of the image become fragile. The most stable and recoverable places in the image in a distorted situation are the low- or high-frequency bands. If binary values are flipped, log (0) becomes negative infinity based on \ref{eq:cross_entropy}. 

\begin{equation}
    \mathcal{L}_{CE}
    = 
    - \sum_{i}
    \left(
        y_i \, \log(p_i)
        +
        (1 - y_i)\,\log(1 - p_i)
    \right)
    \label{eq:cross_entropy}
\end{equation}

To ensure CE does not explode, the encoder must provide predictable structures and that is only possible in high or low-frequency bands. However, these bands are mostly outside of the visual spectrum. Thus, UnMarker can distort these frequencies while maintaining the visual constraint of Perceptual Loss (explained in detail later). UnMarker distorts these spectral amplitudes aggressively and as a result, the decoder only receives junk probabilities, rendering the watermarks useless.

\paragraph{Learned perceptual image patch similarity loss}
Perceptual Loss, formally known as the Learned Perceptual Image Patch Similarity Loss (LPIPS), is a measure of the difference between two images from a human's point of view. Humans do not notice change in pixel values. The same can also be mentioned about Convolutional Neural Networks (CNN)  view images to similarly to humans. The kernels extract feature maps to learn edges, shapes and textures within the edge to view the image like humans view the image. LPIPS loss is crucial for both WMs and UnMarker as it enables image modifications with constraints to attacks and defensive mechanisms that enable changes within the image while ensuring minimal visual changes.

Images are passed through deep CNNs, typically VGG or AlexNet. Each layer $l$ outputs feature maps $\phi_l(\cdot)$ where shallow layer maps consists of edges and as it goes deeper, the layers learn and output feature maps that goes in this order, edges - textures - pattern - shape - full image with all attributes. Hence, the CNN is expected to learn what the human eyes learn after the output of the feature maps from final layers.

The above mentioned process is computed for both original and watermarked images. Afterwards, LPIPS compares the feature maps (sigma) of the original image $I$ and the watermarked image $I_{WM}$ using Equation \ref{eq:lpips_basic}. This is crucial as feature maps can be similar while pixel values within are changed. WMs use this for embedding their signatures and UnMarker further activates LPIPS constraints to disrupt locations where these signatures may be embedded.

\begin{equation}
    \text{LPIPS}(I, \hat{I})
    =
    \sum_{l}
    w_{l} \,
    \Big\|
        \hat{\phi}_{l}(I) - \hat{\phi}_{l}(\hat{I})
    \Big\|_{2}^{2}
    \label{eq:lpips_basic}
\end{equation}

The full breakdown of how LPIPS works is shown in Equation \ref{eq:lpips_full}. LPIPS computes visual differences by comparing the feature maps at each spatial location $(h,w)$ across all convolutional layers. The step-by-step process is given below after the equation.

\begin{equation}
\resizebox{0.90\columnwidth}{!}{$\displaystyle
    \text{LPIPS}(I, \hat{I})
    =
    \sum_{l}
    \frac{1}{H_l W_l}
    \sum_{h=1}^{H_l}
    \sum_{w=1}^{W_l}
    \left\|
        w_{l} \odot 
        \left(
            \hat{\phi}_{l}(I)_{} -
            \hat{\phi}_{l}(\hat{I})_{hw}
        \right)
    \right\|_{2}^{2}
$}
    \label{eq:lpips_full}
\end{equation}

\begin{enumerate}
    \item \textbf{Spatial averaging}: $\frac{1}{H_l W_l}$ in Equation \ref{eq:lpips_full} normalizes the feature maps of size $H_l \times W_l$ by averaging the perceptual loss across all  spatial locations $(h,w)$. This ensures that larger feature maps do not dominate the loss functions and smaller feature maps and every layer contributes to the final spatial distance.
    
    \item \textbf{Channel-wise weighting}: Element-wise matrix multiplication $w_l \odot (\cdot)$ is computed channel wise using the learned weight vector $w_l$. These weights compute the perceptual importance of each feature channel and are determined during training. This ensures that features maps, which are more relevant to humans (edges, textures, shapes), contribute more strongly.
    
    \item \textbf{Feature normalization}: Feature maps are normalized to unit length and represented by $\hat{\phi}_l(\cdot)$. This forces LPIPS to focus more on direction than magnitude of feature maps, emphasising structural elements (texture and edge) over pixel intensity. This aligns LPIPS to human perception.
\end{enumerate}

The above-mentioned method is critical for watermarking methods. Successful WM needs to be invisible to the human eye, of good quality and robust to distortions. LPIPS constraints ensure structural elements of the image remain the same when WM embeds its signature, as shown in Equation \ref{eq:lpips_wm_min}. Loss Functions like MSE significantly penalize the images if pixel values differ, even if they are invisible to the human eye. LPIPS tackles these limitations and enables large changes as long as they are not visible.


\begin{equation}
    \theta_{\text{WM}}^{*}
    =
    \arg\min_{\theta_{\text{WM}}}
    \; \mathcal{L}_{\text{LPIPS}}^{\text{WM}}
    =
    \arg\min_{\theta_{\text{WM}}}
    \; \text{LPIPS}(I, I_{\text{WM}})
    \label{eq:lpips_wm_min}
\end{equation}

However, for all these above-mentioned reasons, LPIPS also has weaknesses that UnMarker can exploit. LPIPS is blind to high-frequency changes. Furthermore, it is blind to the alteration of spectral amplitudes, which enables high-frequency distortion (Cross Entropy) within the image. This further allows distortion of watermarker signatures. This is exactly what the UnMarker uses. The UnMarker attacks in frequency space, modifies amplitudes and adds tiny pixel noise. All of these are designed to target the disruption of WM signal. The UnMarker uses LPIPS to do this as shown in Equation \ref{eq:lpips_unmarker_full}. They compare the LPIPS error and as long as the LPIPS error is under the threshold. UnMarker causes maximum distortion of the image in regions where the watermark is most likely to be present and attacks it aggressively. The result is changes within the spectral amplitudes of the image; the watermark is removed while the visual changes are negligible.

\begin{equation}
\resizebox{0.90\columnwidth}{!}{$\displaystyle
    \text{LPIPS}\big(I_{\text{WM}}, I_{A}\big)
    =
    \sum_{l}
    \frac{1}{H_l W_l}
    \sum_{h=1}^{H_l}
    \sum_{w=1}^{W_l}
    \left\|
        w_{l} \odot
        \big(
            \hat{\phi}_{l}(I_{\text{WM}})_{hw}
            -
            \hat{\phi}_{l}(I_{A})_{hw}
        \big)
    \right\|_{2}^{2}
$}
    \label{eq:lpips_unmarker_full}
\end{equation}


\subsubsection{Fourier basics}
The Fourier Transform (FT) is a mathematical operation used to convert signals from the spatial domain into the frequency domain. Images are considered two-dimensional signals for FTs. FTs break down images using pixel intensities into a set of sinusoidal functions with varying frequencies. Thus, instead of looking at images as a grid of pixel values, FTs view images as a combination of varying low-frequency, medium-frequency, and high-frequency signals. Each of these signals (sinusoidal waves) have frequency (speed of the signal) and amplitude (size of the signal).

For a grayscale image $I(x,y)$ of width $W$ and height $H$, the two-dimensional 
Discrete Fourier Transform (DFT) is defined as shown in Equation \ref{eq:2d_dft}, where $(u,v)$ represents the frequency coordinates and $F(u,v)$ is the frequency 
representation of the image.

\begin{equation}
    F(u,v) =
    \sum_{x=1}^{H}
    \sum_{y=1}^{W}
    I(x,y)\,
    e^{-j 2 \pi \left( \frac{ux}{H} + \frac{vy}{W} \right)}
    \label{eq:2d_dft}
\end{equation}

For RGB images, with multiple channels, the same equation needs to be applied independently across each channel $c \in \{R, G, B\}$ as shown in Equation \ref{eq:2d_dft_rgb}



\begin{equation}
\resizebox{0.90\columnwidth}{!}{$\displaystyle
    F_c(u,v) =
    \sum_{x=1}^{H}
    \sum_{y=1}^{W}
    I_c(x,y)\,
    e^{-j 2\pi \left( \frac{ux}{H} + \frac{vy}{W} \right)},
    \qquad c \in \{R, G, B\}.
$}
    \label{eq:2d_dft_rgb}
\end{equation}

The example of low and high frequency in relation to pixel values is given below. Edges represent high frequency and centers of an object represent low frequencies.

Low-Frequency Example - When the pixel values are very similar, they will be represented by low-frequency FT signals where the differences are small and transitions are smooth. These represent small textures and large shapes within the image.
\[
\begin{bmatrix}
120 & 122 & 123 & 125 \\
121 & 123 & 124 & 126 \\
122 & 123 & 125 & 127 \\
123 & 124 & 126 & 128
\end{bmatrix}
\]


High-Frequency Example - When the pixel values change rapidly and sharply, they represent high-frequency components in the image. 
For example, consider a region with alternating intensities as shown below. These high-frequency signals represent edges, textures and transition areas within the image

\[
\begin{bmatrix}
0 & 255 & 0 & 255 \\
255 & 0 & 255 & 0 \\
0 & 255 & 0 & 255 \\
255 & 0 & 255 & 0
\end{bmatrix}
\]

WM schemes typically add tiny patterns within these high frequencies which are beyond the visual spectrum of humans. Sometimes, techniques like TRW also add stable patterns to low frequencies that the decoder can decode. However, the UnMarker uses these same techniques to add noise to these high and low patterns, so the decoder of WM is rendered useless.

The mathematical derivation of this is provided below. FT components of an each can be further decomposed into two elements:
\[
F(u,v) = |F(u,v)| \, e^{j \angle F(u,v)},
\]
\textbf{Magnitude} represents the strength of each frequency denoted by $|F(u,v)|$. \textbf{Phase} represents the location of objects in the image denoted by $\angle F(u,v)$ 



Changes in magnitude do not significantly alter the image. However, small changes in the phase completely distort the image. Hence, WM schemes must hide their contents within the magnitude. The phase is unchanged to preserve shape, edge, and object position. Hence, typical WM schemes for the Fourier Transformation to embed a digital signature can be shown in Equation \ref{eq:wm_magnitude_embedding}.

\begin{equation}
    |\widetilde{F}(u,v)|
    =
    |F(u,v)| \; + \; \alpha \, W(u,v),
    \label{eq:wm_magnitude_embedding}
\end{equation}

Where:
\begin{itemize}
    \item $F(u,v)$ — original Fourier coefficient.
    \item $|F(u,v)|$ — original magnitude of the Fourier coefficient.
    \item $W(u,v)$ — watermark pattern embedded in the frequency domain.
    \item $\alpha$ — embedding strength.
    \item $|\widetilde{F}(u,v)|$ — watermarked magnitude after embedding.
\end{itemize}

Based on the above scheme of the WMs, it is understood that the WMs alter the magnitude spectrum $|F(u,v)|$ in both high and low-frequency signals. The alteration needs to be predictable to ensure that WM decoders can decode it. This is exactly what the UnMarker uses to its advantage. UnMarker targets the frequency ranges that hide these signals and maximizes distortion in those locations. The UnMarker follows the same route as the WM schemes. They keep the phase component $\angle F(u,v)$ unchanged so the image remains the same visually. Then UnMarker aggressively attacks the low and high frequency components $|F(u,v)|$. The paper introduces the Direct Fourier Loss (DFL) as shown in Equation \ref{eq:dfl}. The DFL measures the difference between the Fourier magnitudes of the attacked image $|F_{\text{A}}(u,v)|$ and watermarked image $|F_{\text{WM}}(u,v)|$. UnMarker aims to maximize this operation using the notation shown in Equation \ref{eq:dfl_max}. This is one of the three main components of the UnMarker optimization as shown in Equation \ref{eq:unmarker_full_loss}

\begin{equation}
    \mathcal{L}_{\text{DFL}}
    =
    \sum_{u,v}
    \left(
        |F_{\text{WM}}(u,v)| -
        |F_{\text{A}}(u,v)|
    \right)^{2}
    \label{eq:dfl}
\end{equation}


\begin{equation}
    \theta^{*}
    =
    \arg\max_{\theta}
    \; \mathcal{L}_{\text{DFL}}(\theta)
    \label{eq:dfl_max}
\end{equation}


\begin{equation}
    \mathcal{L}_{\text{UnMarker}}
    =
    \lambda_{\text{DFL}} \, \mathcal{L}_{\text{DFL}}
    +
    \lambda_{\text{LPIPS}} \, \mathcal{L}_{\text{LPIPS}}
    +
    \lambda_{\text{TV}} \, \mathcal{L}_{\text{TV}}.
    \label{eq:unmarker_full_loss}
\end{equation}

\subsubsection{Convolution basics}
Convolution is a fundamental operation of image processing. Convolution involves passing a mathematical matrix (also known as a kernel) pixel by pixel through the whole image to identify patterns. The type of pattern found is determined by the type of kernel. An image can be passed through multiple kernels to find the desired patterns within the image. This operation is the core idea upon which state-of-the-art Convolutional Neural Networks are built. The field of computer vision is now heavily reliant on convolution operations.


The convolution for two continous functions $f(t)$ and $g(t)$ is shown in Equation \ref{eq:continuous_convolution}. Here, $*$ is the convolution operation. The first function is shifted, reversed and then multiplied pointwise by the second function. Discrete one-dimensional convolution is shown in Equation \ref{eq:discrete_convolution_1d}. Images are typically two-dimensional. The image and 2D convolution are shown in Equation \ref{eq:discrete_convolution_2d}. Here, $(m,n)$ indicates the spatial location of the output image. During implementation, cross-correlation is used over convolution due to ease in implementation and is shown in Equation \ref{eq:cross_correlation}. The $\star$ refers to cross-correlation. Reversing the kernel is not required in cross-correlation and is used as a convolution layer in CNN.

\begin{equation}
(f * g)(t) = \int_{-\infty}^{\infty} f(\tau)\, g(t-\tau)\, d\tau
\label{eq:continuous_convolution}
\end{equation}


\begin{equation}
(f * g)[n] = \sum_{k=-\infty}^{\infty} f[k]\, g[n-k]
\label{eq:discrete_convolution_1d}
\end{equation}


\begin{equation}
(I * K)[m,n] = \sum_{i}\sum_{j} I[i,j]\, K[m-i, n-j]
\label{eq:discrete_convolution_2d}
\end{equation}




\begin{equation}
(I \star K)[m,n] = \sum_{i}\sum_{j} I[m+i, n+j]\, K[i,j]
\label{eq:cross_correlation}
\end{equation}


In convolution, a square kernel is passed across the image, computing the product of the kernel values and corresponding pixel values. Afterwards, the products are summed to a single output value. The single values represent one pixel in the output feature map. The kernel then moves one stride to the next pixel until the same operation is completed over the entire image. The output is the convolved image of the input image. The outputs represent specific patterns such as edges, textures, smooth lines, and shapes based on the kernel. For illustration below a a $5 \times 5$ grayscale image is considered below alongside a simple $3 \times 3$ edge-detection kernel:

\[
I =
\begin{bmatrix}
 10 & 10 & 10 & 10 & 10 \\
 10 & 10 & 10 & 10 & 10 \\
100 & 100 & 100 & 100 & 100 \\
100 & 100 & 100 & 100 & 100 \\
100 & 100 & 100 & 100 & 100
\end{bmatrix}
\]

\[
K =
\begin{bmatrix}
-1 & -1 & -1 \\
 0 &  0 &  0 \\
 1 &  1 &  1
\end{bmatrix}
\]

With a stride (step-size) of 1, the output is a 3 by 3 feature map that detects horizontal edges as shown below:

\[
\text{Output Feature Map} =
\begin{bmatrix}
270 & 270 & 270 \\
270 & 270 & 270 \\
0   & 0   & 0
\end{bmatrix}
\]

From the above, it can be seen that the output map strongly detects the edge between the second and third rows. Hence, convolution is extremely important for watermarking. These are not only spatial filters. The Convolution Theorem states that convolution is equivalent to multiplication in the Fourier domain. Hence, each kernel represents a specific frequency response. The following kernels relevant to watermarkers and UnMarker, due to their abilities to modify the frequency components of the image, are provided below:

\begin{itemize}

    \item High-pass filtering (edge detection):  
    These filters enhance high-frequency components such as edges.  
    Example kernel:
    \[
    K_{\text{edge}} =
    \begin{bmatrix}
    -1 & -1 & -1 \\
     0 &  0 &  0 \\
     1 &  1 &  1
    \end{bmatrix}
    \]

    \item Laplacian filtering (second-order edge detection):  
    Highlights rapid intensity changes across all directions.  
    Example kernel:
    \[
    K_{\text{laplace}} =
    \begin{bmatrix}
     0 & -1 &  0 \\
    -1 &  4 & -1 \\
     0 & -1 &  0
    \end{bmatrix}
    \]

    \item Low-pass filtering (smoothing/blur):  
    Removes high-frequency detail such as noise and fine texture.  
    Gaussian blur kernel:
    \[
    K_{\text{gauss}} = \frac{1}{16}
    \begin{bmatrix}
    1 & 2 & 1 \\
    2 & 4 & 2 \\
    1 & 2 & 1
    \end{bmatrix}
    \]

    \item Mean filter (simple blur):  
    Averages local neighborhoods to reduce noise.  
    \[
    K_{\text{mean}} = \frac{1}{9}
    \begin{bmatrix}
    1 & 1 & 1 \\
    1 & 1 & 1 \\
    1 & 1 & 1
    \end{bmatrix}
    \]

    \item Sharpening filter (high-boost filtering):  
    Enhances edges and fine detail by amplifying high frequencies.  
    Example kernel:
    \[
    K_{\text{sharpen}} =
    \begin{bmatrix}
     0 & -1 &  0 \\
    -1 &  5 & -1 \\
     0 & -1 &  0
    \end{bmatrix}
    \]

    \item Median filtering:  
    A non-linear filter replaces each pixel with the median of its neighborhood.  

    \item Bilateral filtering:  
    Smooths textures while preserving edges by weighting pixels based on both 
    spatial distance and intensity similarity.  
    \[
    \resizebox{0.98\linewidth}{!}{$\displaystyle
    I'(x,y) = 
    \frac{
        \sum_{i,j} I(i,j)\,f_s(\lVert (i,j)-(x,y)\rVert)\,f_r(|I(i,j)-I(x,y)|)
    }{
        \sum_{i,j} f_s(\lVert (i,j)-(x,y)\rVert)\,f_r(|I(i,j)-I(x,y)|)
    }
    $}
    \]

    \item CNN learned filters:  
    Convolutional neural networks learn their own kernels to detect patterns such as edges, textures, and shapes. 

\end{itemize}


\subsubsection{Convolution in watermarks and UnMarker}
Watermarks use the above-mentioned methods to embed their digital signatures under LPIPS constraints (explained above). Based on convolution filters, low-frequency regions represent global structures like colours, transitions and shapes. Changing these structures becomes easily visible and breaks the LPIPS constraints. Hence, low filter embedding of digital signatures is difficult (StegaStamp and TRW are the exceptions). Watermarks, therefore, hide their signature in most cases in high-frequency regions

StegaStamp uses a spatial transformer network to embed the signature in low and mid-frequency components. The network uses convolution layers to learn smooth and stable distortion patterns. They embed the distortions here to ensure the WM remains stable under real-world distortions (cropping). Tone-Residual Watermarking (TRW) modifies moderate frequency components, making it resistant to downscaling and compression. It uses convolution to find smooth brightness patterns. The signature is mostly embedded by slight changes of color channels and low-frequency brightness settings. The decoder uses convolutional filters to read these changes.

In high frequency, more changes can be made by the WMs. However, these methods are fragile to simple distortions. HiDDeN uses an encoder CNN to find high-frequency textures and add noise.  The decoder is trained alongside to learn these patterns. PTW breaks images into patches and runs convolution filters on them. It embeds its signatures in the high-frequency patches that only its detector knows. Stable Signature uses diffusion models that produce high-frequency content. CNNs detect high-frequency regions and inject consistent WM patterns.


The UnMarker knows that WM uses CNN-based decoders to read the patterns. Hence, UnMarker disrupts both low and high frequency patterns with two types of attacks. Watermark decoders rely on the consistency of these feature maps to detect the watermark pattern.
\begin{itemize}
    \item Non-Semantic watermarks: These are the high-frequency watermarks. For non-semantic attacks, UnMarker targets shallow convolution layers as they target high-frequency features. UnMarker modifies the image so that the difference between shallow feature maps between the watermarked image $I_\text{WM}$ and the attacked image $I_A$ is maximized,

\[
\| f_{1}(I_{\text{WM}}) - f_{1}(I_{A}) \|_{2} \text{ is maximised},
\]

while keeping $I_{A}$ visually close to $I_{\text{WM}}$ (LPIPS constraint). This disrupts the decoder's ability to decode the signatures of WM.
    \item Semantic watermarks: These are the low-frequency watermarks. For semantic attacks, UnMarker targets the deeper convolution layers whose feature maps represent stable patterns. UnMarker increases the difference between the feature maps of the watermarked image $I_\text{WM}$ and the attacked image $I_A$. In the equation below, $L$ refers to deep convolution layers. Again, the decoder fails to detect these signatures after minor distortions, as the signatures in low frequencies are very slight adjustments anyway.

\[
\| f_{L}(I_{\text{WM}}) - f_{L}(I_{A}) \|_{2} \text{ to increase},
\]
\end{itemize}

Therefore, based on the above, UnMarkers disruption of feature maps can be provided using the equation \ref{eq:unmarker_semantic_nonsemantic}, subject to LPIPS constraints.

\begin{equation}
    \max_{\theta} 
    \left(
        \alpha \, \| f_{1}(I_{\text{WM}}) - f_{1}(I_{A}) \|_{2}
        +
        \beta \, \| f_{L}(I_{\text{WM}}) - f_{L}(I_{A}) \|_{2}
    \right)
    \label{eq:unmarker_semantic_nonsemantic}
\end{equation}
\noindent Where:
\begin{itemize}
    \item $f_{1}(\cdot)$: low-level feature maps.
    \item $f_{L}(\cdot)$: high-level feature maps.
    \item $I_{\text{WM}}$: watermarked image.
    \item $I_{A}$: attacked image.
    \item $\alpha$: coefficient to represent the strength of non-semantic/ high frequency / shallow layer attacks. 
    \item $\beta$: coefficient to represent the strength of semantic attack / low-frequency / deeper layer attacks.
    \item $\theta$: learnable parameters of the UnMarker distortions.
\end{itemize}

\subsubsection{Constrained optimization}

Constraint Optimization in mathematics refers to the best possible solution while respecting certain limitations. Considering the scenario of watermarking and watermark removal, certain aspects of the image require change while the image remains virtually the same. Therefore, in the case of watermarking, LPIPS is the constraint and within these constraints, maximal encoding needs to be performed. Therefore, the goal is to encode the signature. The constraint is that the image looks the same. This can be shown in Equation \ref{eq:constraint_basic}.

\begin{equation}
    \max_{\theta} \; \mathcal{C}(\theta)
    \quad \text{subject to} \quad 
    \text{image\_looks\_same} \; or (I, I_{\theta}) \leq T,
    \label{eq:constraint_basic}
\end{equation}

\noindent Where:
\begin{itemize}
    \item $\theta$ represents the parameters controlling the modification applied to the image.
    \item $\mathcal{C}(\theta)$ is the watermark embedding being maximised.
    \item $I$ is the original image.
    \item $I_{\theta}$ is the watermarked image after applying the transformation $\theta$.
    \item $T$ is the LPIPS constraint for visual change limitation
\end{itemize}

In mathematical optimization, an objective is to be maximized or minimized. Directly solving such problems under constraints is difficult. Therefore, Lagrangian proposes a powerful method to solve optimization problems. The Lagrangian introduces a new variable called the Lagrangian multiplier $\lambda \ge 0$. Using $\lambda \ge 0$, the expression can be combined into a single expression.

\[
\mathcal{L}(\theta, \lambda)
=
f(\theta) + \lambda \, g(\theta).
\]

The idea is that when the constraint term is violated( i.e., $g(\theta) > 0$), the $\lambda g(\theta)$ becomes positive and acts as a penalty term to penalize the objective. The penalty term is 0 when the constraint remains satisfied and the solution can focus on maximizing the objective $f(\theta)$. Thus, the Lagrangian is a powerful tool for converting a constrained optimization into an unconstrained standard optimization problem. For the constraint $\| I - I_{\theta} \| - T \le 0$, the Lagrangian can be written as shown in Equation \ref{eq:wm_lagrangian}

\begin{equation}
    \mathcal{L}_{\text{WM}}(\theta, \lambda)
    =
    \mathcal{C}_{\text{WM}}(\theta)
    +
    \lambda \left( T - \| I - I_{\theta} \| \right),
    \label{eq:wm_lagrangian}
\end{equation}

The next step is to determine whether the solution is optimal or not. For an optimal solution, the Karush-Kuhn-Tucker (KKT) conditions provide the requirements for a solution in constrained optimization. In an optimal solution, $\theta = \theta^{*}, \space
\lambda = \lambda^{*}$.

The UnMarker behaves in the same way as WM methods for constrained optimization. Here, the goal is to maximize change in frequency content, also known as spectral disruption, such that the image still looks the same. This can be represented with the Direct Fourier Loss as shown in Equation \ref{eq:dfl_max}. Therefore, the constraint optimization based on the above is shown in Equation \ref{eq:unmarker_constraint}.

\begin{equation}
    \max_{\theta} \; \mathcal{L}_{\text{DFL}}(\theta)
    \quad \text{subject to} \quad
    (I_{\text{WM}} - I_{A}(\theta)\big) \leq T,
    \label{eq:unmarker_constraint}
\end{equation}

Therefore, the Lagrangian of  UnMarker is shown in Equation \ref{eq:unmarker_lagrangian}.


\begin{equation}
\resizebox{0.90\columnwidth}{!}{$\displaystyle
    \mathcal{L}_{\text{UM}}(\theta, \lambda)
    =
    \mathcal{L}_{\text{DFL}}(\theta)
    +
    \lambda
    \left(
        T
        -
        \text{LPIPS}\big(I_{\text{WM}}, I_{A}(\theta)\big)
    \right),
    \quad \lambda \ge 0,
$}
    \label{eq:unmarker_lagrangian}
\end{equation}
\noindent Where:
\begin{itemize}
    \item $\mathcal{L}_{\text{DFL}}(\theta)$ is the Direct Fourier Loss, measuring
    spectral disruption between the watermarked and attacked image.
    \item $\text{LPIPS}\big(I_{\text{WM}}, I_{A}(\theta)\big)$ is the perceptual distance
    between the watermarked image $I_{\text{WM}}$ and the attacked image $I_{A}(\theta)$.
    \item $T$ is the maximum allowed perceptual change.
    \item $\lambda$ is the Lagrangian multiplier enforcing the perceptual constraint.
\end{itemize}

From the above points, it can be understood that for constrained optimization, Watermarker and UnMarker have the same constrained optimization problem with the opposite objective. Watermarkers aim to maximize embedding strength, while UnMarker maximizes the spectral disruption of the embedding. However, the UnMarker has a unique advantage. Watermarker methods operate with perceptual constrains and preserve stable structures so that the decoder can recover the signatures and read them. UnMarker has no such issues, as they deliberately target and cause maximum destruction to these structures. LPIPS is blind to these high-frequency changes; UnMarker can introduce large spectral changes within the perceptual limit.

The constraints also severely limit where watermarks can actually hide, pushing WMs to be embedded in predictable regions. In the next section, HiDDeN, the first deep learning based watermarking scheme, is introduced. Later on, it introduces a weakness that is directly related to these constraints.

\subsection{{HiDDeN}}
HiDDeN \cite{zhu2018hidden} is the first deep learning-based, robust and invisible watermarking scheme introduced in 2018. This algorithm serves as the building block for later watermarking schemes discussed in this section. HiDDeN uses a neural network to embed its signature in images such that the image remains imperceptible. Yet, the HiDDeN decoder can recover the signal even after it undergoes common distortions. Overview of HiDDeN is shown in Figure \ref{fig:hidden_overview}. The architecture can be broken down to four main components: The \textbf{Encoder}, a \textbf{Noise Layer}, the \textbf{Decoder}, and an \textbf{Adversarial Discriminator}. In this section, first the \textbf{Loss Functions} are discussed, followed by the four main components in depth. Finally, the iterative \textbf{Optimization Loop} shows how the components interact with each other. In short, the Encoder is tasked with encoding the message within the image. The Noise Layer then adds random noise mimicking real-life scenarios that the watermarked image may go through. The Decoder's objective is to retrieve the message from the Encoder after distortions. Finally, the Adversarial Discriminator is used to predict the output of the Encoder (and Decoder) to see if it can successfully detect watermarked images. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/HiDDeN.png}
    \caption{Overview of the HiDDeN watermarking framework. Source: adapted from \cite{zhu2018hidden}.}
    \label{fig:hidden_overview}
\end{figure}

\subsubsection{Loss functions}
During training, the encoder and decoder are trained simultaneously to minimize the sum of the three losses, \textbf{Message Reconstruction Loss}, \textbf{Image Distortion Loss}, and \textbf{Total Loss}. The Discriminator Loss classifies the output of the encoder, and it is minimized during training.


\paragraph{Message Reconstruction loss}
Message Reconstruction Loss (MRL), denoted as $L_M$, is the decoder's loss function. MRL computes how well the decoder decodes the initial message $M_{\text{in}}$ provided to the Encoder. MSE is used to compute the error between the original bits $M_{\text{in}}$ and the decoder's output $M_{\text{out}}$ as shown in the equation \ref{eq:mrl}.
\begin{equation}
    L_{M}(M_{\text{in}}, M_{\text{out}})
    =
    \frac{1}{L}
    \left\|
        M_{\text{in}} - M_{\text{out}}
    \right\|_{2}^{2},
    \label{eq:mrl}
\end{equation}

The goal is to minimize $L_M$ to ensure the decoder learns to extract the message embedded by the encoder. Ideally, $L_M=0$ if $M_\text{in}$ is reconstructed perfectly.

\paragraph{Image distortion loss}
The Image Distortion Loss (IDL) used in hidden is the same MSE discussed in Equation \ref{eq:mse_watermarking}. The mathematical expression is identical and it is used during training to penalize visible differences between the original image $I$ and the watermarked image $I_\text{WM}$. The loss ensures that visually identical images are produced.
\paragraph{Adversarial loss}
Adversarial Loss is derived from the discriminator’s prediction. This is the final component of the encoder's loss. The $L_G$ encourages the encoder to produce output images that cannot be correctly classified by the Discriminator. Therefore, the encoder is attempting to fool the Discriminator from understanding that bit messages are hidden inside the image. The adversarial loss used in HiDDeN is defined in Equation \ref{eq:adv_loss}.
\begin{equation}
    L_G(I_{\text{en}})
    =
    \log\!\left( 1 - A(I_{\text{en}}) \right),
    \label{eq:adv_loss}
\end{equation}
where $A(I_{\text{en}})$ is the discriminator's probability that the image is watermarked with the message $I_{\text{en}}$. Thus, minimizing $L_G$ makes $A(I_{\text{en}})$ decrease to $0$ as the discriminator fails to classify the image.
\paragraph{Discriminator loss}
The Discriminator Loss (DL) determines the discriminator's ability to distinguish between the cover image/original image $I_{co}$ and 
encoded images $I_{en}$. The loss function is defined in Equation \ref{eq:disc_loss}.

\begin{equation}
    L_A(I_{co}, I_{en})
    =
    -\Big[
        \log\big(1 - A(I_{co})\big)
        +
        \log\big(A(I_{en})\big)
      \Big],
    \label{eq:disc_loss}
\end{equation}
The discriminator minimizes $L_A$  w.r.t. the parameter $\gamma$. The term $\log\big(1 - A(I_{co})\big)$ penalizes when the cover image is predicted as the encoded image and vice versa for $\log\big(A(I_{en})\big)$. The encoder indirectly maximizes $L_A$ by minimizing $L_G$.

\paragraph{Total loss}
The encoder and decoder together form the hidden network. They optimize a weighted sum of the losses as shown in Equation \ref{eq:total_encdec}.

\begin{equation}
\resizebox{0.90\columnwidth}{!}{$\displaystyle
    \mathcal{L}_{\text{Enc+Dec}}(\theta,\phi)
    =
    L_{M}\big(M_{\text{in}}, D_{\phi}(I_{\text{en}})\big)
    +
    \lambda_{I}\, L_{I}\big(I, I_{\text{en}}\big)
    +
    \lambda_{G}\, L_{G}\big(A_{\gamma}(I_{\text{en}})\big),
$}
    \label{eq:total_encdec}
\end{equation}
\noindent Where:
\begin{itemize}
    \item $I_{\text{en}} = E_{\theta}(I, M_{\text{in}})$ is the encoded image.
    \item $L_{M}(M_{\text{in}},M_{\text{out}}) = \frac{1}{L}\|M_{\text{in}} - M_{\text{out}}\|_2^{2}$ is the message reconstruction loss.
    \item $L_{I}(I, I_{\text{en}}) = \| I - I_{\text{en}} \|_2^{2}$ is the image distortion loss.
    \item $L_{G}(I_{\text{en}}) = \log\left(1 - A_{\gamma}(I_{\text{en}})\right)$ is the adversarial loss.
    \item $\lambda_{I}$ is the coefficient that controls image modification.
    \item $\lambda_{G}$ is the coefficient that controls how strongly the encoder acts to fool the discriminator. 
\end{itemize}
$\lambda_I$ and $\lambda_G$ act similarly to Lagrangian multipliers, explained earlier in Constrained Optimization. Here, $\lambda_{I}$ controls the visual changes allowed by the encoder and keeps the encoded image $I_{\text{en}}$ perceptually similar to $I$. Decreasing $\lambda_I$ will allow more visible distortion. $\lambda_{G}$ controls how strongly the encoder tries to fool the discriminator. Hence, a higher $\lambda_{G}$ enforces adversarial stealth, making it more difficult to detect by the discriminator, consequently also more difficult for external detectors.

The discriminator is trained with a separate objective as shown in Equation \ref{eq:total_loss_disc}.
\begin{equation}
    \mathcal{L}_{\text{Disc}}(\gamma)
    =
    -\Big[
        \log\big(1 - A_{\gamma}(I_{co})\big)
        +
        \log\big(A_{\gamma}(I_{\text{en}})\big)
      \Big],
    \label{eq:total_loss_disc}
\end{equation}

During training, optimization alternates between the encoder-decoder parameters and the discriminator parameters. During encoder-decoder optimization $(\theta,\phi)$ are updated to minimize $\mathcal{L}_{\text{Enc+Dec}}$. In the next step, $\gamma$ is updated to minimize 
$\mathcal{L}_{\text{Disc}}$. This alteration results in watermarks being embedded into high-frequency components of the image. $L_I$ penalizes large changes in pixel values, and so modifications in pixel values are small and subtle. $L_G$ ensures modifications seem natural in the image. $L_M$ ensures watermarks are strong enough to be decoded after distortions.
   
\subsubsection{Encoder}
In HiDDeN, the encoder $E_{\theta}$ is tasked with hiding the binary message $M_{\text{in}} \in \{0,1\}^{L}$ of length $L$ within the cover image $I_{co} \in \mathbb{R}^{C \times H \times W}$. Thus, the encoder is a CNN that takes as input the binary message and the cover image. The encoder embeds the message into the image and the output is an encoded image $I_{\text{EN}} \in \mathbb{R}^{C \times H \times W}$, also known as the stego image. The stego image has the same dimensions as the original image/cover image so that the embedding does not change the image resolution or format. The encoder learns to embed the message in the image using the following Equation \ref{eq:encoder_delta}. Here, the encoder learns the embedding $\Delta I \in \mathbb{R}^{C \times H \times W}$ and encodes it within the image while remaining visually indistinguishable from the cover image $I_{co}$.


The encoder is designed to embed the message $M_{in}$ gradually within the spatial features of the image $I_{co}$. Initially, $I_{co}$ is passed through shallow convolution layers to extract low and mid-level feature representations $f$. These are typically edges and textures within the image. Afterwards, $M_{in}$ is replicated to match the dimensions of $f$. The replicated version of $M_{in}$ is concatenated to the image along the channel dimension. Therefore, each spatial dimension of the image has access to $M_{in}$. During further convolution operations, the filter can notice $M_{in}$ as they traverse through the pixel grids of the concatenated image. Encoding with the feature maps enables the encoder to embed the message across the whole spatial dimension of the image.

\begin{equation}
    I_{\text{EN}} = I_{co} + \Delta I,
    \label{eq:encoder_delta}
\end{equation}

The image is then passed through more convolutional layers to refine the stego image further. The deeper layers learn to embed $M_{in}$ while preserving visual quality during optimization iterations. The final layer outputs the refined image $I_{en}$.


The encoder needs to embed in such a way that $I_{en}$ remains indistinguishable from $I_{co}$ while keeping $M_{in}$ recoverable for the decoder. In the frequency domain using the Fourier knowledge, indistinguishability implies that the dominant 
low-frequency components capture global structures, brightness, and smooth regions. These cannot have a significant impact. Therefore, the encoder is limited to preserving the low-frequency magnitude of the image’s Fourier transform.

Furthermore, recovering $M_{in}$ requires the embedding signal $\Delta F$ to be robust to 
distortions. Thus, the encoder naturally modifies high-frequency components that capture textures and edges. These are mostly beyond human perception, but 
can be detected by the decoder. The term in the Fourier domain is shown in Equation \ref{eq:encoder_frequency} below. Hence, HiDDeN watermarks appear noise-like and are especially vulnerable to attacks that distort high-frequency ranges.

\begin{equation}
    F_{\text{EN}}(u,v) = F_{co}(u,v) + \Delta F(u,v),
    \label{eq:encoder_frequency}
\end{equation}

\subsubsection{Decoder}
The decoder $D_{\phi}$ is designed to extract  $M_{\text{in}} \in \{0,1\}^{L}$ of length $L$ that was provided as input and embedded in encoded image $I_{en}$. The input of the decoder is the $I_{en}$ alongside an added noise to form $I_{no}$ as shown in Equation \ref{eq:noise_addition}. $N(\cdot)$ is the noise added in the noise layer discussed in the next subsection.


For training purposes, the decoder is provided with a noisy version of the image that simulates real-world distortions watermarks may go through. The objective of the decoder is a predicted message $M_{out}$ that replicates $M_{in}$.


The decoder is a CNN similar to the encoder, but in reverse. Firstly, the decoder passes $I_{no}$ through multiple convolution layers to extract feature maps. For each output bit, the decoder collects information from the entire image $I_{no}$. The final convolution layer produces $L$ feature maps, with each map representing one message bit. Global average pooling is then applied to each feature map to average output of all spatial locations. Hence, the output is an $L$ vector that represents the predicted message $M_{out}$. This architecture ensures the decoder does not assume the watermark is one specific location but rather embedded across the entire image.


The decoder is trained by minimizing the MRL as mentioned in Equation \ref{eq:mrl}. Minimizing $L_M$ ensures the decoder attempts to replicate $M_{in}$. The perfect decoder will have an MRL of 0. However, that is not realistic as decoder outputs are probabilities for each bits while $M_{in}$ is a string of 0 and 1. 

The decoder, average pooling and MRL plays a crucial role as the prediction makes the decoder search for $M_{in}$ across the entire image. During training, this ultimately makes the encoder embed $M_{in}$ across the whole image. This makes the watermark robust to cropping and localized distortions. Therefore, the message is not stored in a single frequency but rather across a range of high-frequency variations across the image. Watermark presence will indicate strong average responses and this enables the decoder to recover the message. This property makes HiDDeN robust to common distortions. However, it also confirms that the watermarks are located in high-frequency contents of the image, which UnMarker later exploits.

\subsubsection{Noise layer}
The Noise layer $N$ is situated between the Encoder-Decoder network and trains them to model and defend against real-world attack simulations. The layer adds controlled distortions of multiple types to the image during training. This ensures that the encoder embeds the message so that it survives distortions. Furthermore, it trains the decoder to recover $M_{in}$. $N$ outputs $I_{no}$ via the representation \ref{eq:noise_addition}.
\begin{equation}
    I_{no} = N(I_{co}, I_{en}),
    \label{eq:noise_addition}
\end{equation}

The types of distortions employed by HiDDeN's noise layer is listed below.
\begin{itemize}
    \item \textbf{Identity:} No change. $I_{no} = I_{en}$. Encoder-Decoder models the clean image.

    \item \textbf{Dropout:} Some pixels of $I_{en}$ are replaced independently with 
    original values from $I_{co}$. All pixels have a random probability to simulate a random loss of embedding.

    \item \textbf{Cropout:} Random region of $I_{en}$ is replaced with $I_{co}$. This simulates partial watermarking strength and trains the decoder to decode.

    \item \textbf{Crop:} This simulates an attacker removing part of the image and resizing it. Portion of $I_{en}$ is cropped out and resized and then added back.
    \item \textbf{Gaussian Blur:} A Gaussian kernel is applied to convolve the image. This distorts high-frequency components and models smoothing.

    \item \textbf{JPEG Compression:} Image is JPEG-compressed. This targets high-frequency components and removes information while also adding compressed noise.
\end{itemize}
Distortions are controlled by intensity to control perturbation strength. During training, a set of the above-mentioned operations are randomly selected and applied to $I_{no}$ to produce $I_{co}$. Among these operations, dropout, crop, and cropout operate in the spatial domain. Gaussian blur and JPEG compression operate in the spatial and frequency domains. This means the embedding must be robust even when parts of the watermark $\Delta F(u,v)$ are distorted or removed completely.
\[
F_{en}(u,v) = F_{co}(u,v) + \Delta F(u,v),
\]
For non-differential operations like JPEG compression, differential approximations are used to enable training backpropagation. This enables the encoder to also learn non-differentiable real-world distortions.
\subsubsection{The adversarial network}
The Adversarial Network idea is also applied in HiDDeN to enforce invisibility of watermarks. The Encoder is the generator and a further Adversarial Discriminator layer $A_{\gamma}$ is used. The Discriminator's role is to differentiate between original and watermarked images. It takes as input an image $\tilde{I}$ and outputs a probability of likelihood that it contains WM as shown below.
\[
A_{\gamma}(\tilde{I}) \in [0,1],
\]

During training, the adversarial optimization process is used. Therefore, in one iteration the Encoder-Decoder is optimized and in next one $A_{\gamma}$ is optimized. This trains the discriminator to correctly predict encoded and non-encoded images. Furthermore, it trains the encoder to generate images that are indistinguishable from non-encoded images.


The architecture of the Discriminator is a CNN similar to the decoder. Image is processed through multiple convolutional layers (feature maps of local textures and global statistics) and then aggregated using global pooling. Afterwards, the maps are sent through an additional sigmoid activation to produce classification probabilities as shown in Equation \ref{eq:sigmoid_disc}. Here, $z$ is the output of the discriminator.
\begin{equation}
    A_{\gamma}(I)
    =
    \sigma(z)
    =
    \frac{1}{1 + e^{-z}},
    \label{eq:sigmoid_disc}
\end{equation}

The shallow convolutional layers enable the discriminator to learn texture and edges. The deeper layer maps represent global patterns. If the encoder consistently makes predictable changes in similar frequency bands, the discriminator will read this and assign high probabilities. The decoder is only trained to learn whether an image is natural or not and is not looking for $M_{out}$.



A competitive objective is used between the Encoder and Discriminator. $A_{\gamma}$ is trained as a binary classifier as shown in Equation \ref{eq:disc_loss}. Minimizing $L_A$ enables the discriminator to learn spectral differences between natural and watermarked images. The encoder is trained with an included adversarial loss component as shown in Equation \ref{eq:adv_loss}. Minimizing $L_G$ indirectly increases $L_A$ by reducing $A_{\gamma}(I_{en})$, which makes it more difficult for the discriminator to correctly predict. This optimization slowly pushes the encoder to hide the image within natural high frequencies of the image that are invisible to humans and difficult for learned detectors to find.
\subsubsection{Optimization loop}
The iterative optimization loop for HiDDeN is shown below.

\begin{itemize}
    \item \textit{Batch selection:}  
    Creates batches of cover images $\{I_{co}\}$ and  binary messages $\{M_{in}\}$ of length $L$ .

    \item \textit{Encoding:}  
    Image–message pair $(I_{co}, M_{in})$ is passed through the encoder 
    $E_{\theta}$ to produce encoded image $I_{en}$. Over time encoder produces images identical to $I_{co}$.   
    \[
    I_{en} = E_{\theta}(I_{co}, M_{in}).
    \]
    \item \textit{Noise simulation:}  
    $I_{en}$ is passed through the noise layer to simulate real-world distortions (from a random set of previously mentioned distortions) to produce $I_{no}$.
    
    \item \textit{Decoding:}  
    Decoder $D_{\phi}$ uses the noised image $I_{no}$ as input and produces a predicted message $M_{out}$
    \item \textit{Discrimination:}  
    Discriminator $A_{\gamma}$ is provided as input cover images $I_{co}$ and 
    encoded images $I_{en}$. It outputs probabilities 
    $A_{\gamma}(I_{co})$ and $A_{\gamma}(I_{en})$ indicating whether each image contains a message.

    \item \textit{Loss computation:}  
    Losses are computed:
    \begin{itemize}
        \item MRL is computed as shown in Equation \ref{eq:mrl}.
        \item IDL is computed as shown in Equation \ref{eq:mse_watermarking}.
        \item Encoder adversarial loss $L_G$ using $A_{\gamma}(I_{en})$ as shown in Equation \ref{eq:total_loss_disc}
        \item Discriminator loss $L_A$ is computed using $A_{\gamma}(I_{co})$ and 
        $A_{\gamma}(I_{en})$ as shown in Equation \ref{eq:disc_loss}
    \end{itemize}

    \item \textit{Encoder–Decoder update:}  
    Alternated optimization of parameters begins. Initial step is the Encoder-Decoder update.
    \begin{enumerate}
        \item The encoder and decoder parameters $(\theta,\phi)$ are updated by minimizing 
    the total loss as shown in Equation \ref{eq:total_encdec}. Gradient Descent-based optimization techniques are used.
        \item \textit{Discriminator Update:}  
    The discriminator parameters $\gamma$ are updated by minimizing the discriminator loss as shown in Equation \ref{eq:disc_loss}.
    \end{enumerate}
    
    \item \textit{Iteration:}  
    Above steps are repeated until convergence. Encoder-Decoder iteratively improves embedding and recovery. Discriminator iteratively adapts to the Encoder generation to detect properly.
\end{itemize}

Convergence occurs when losses stabilize, the discriminator does not improve the classification score, and the decoder retrieves successfully $M_{in}$. At convergence, the encoder-decoder learns robust and invisible watermarks that survives distortion while ensuring message retrieval. Furthermore, the images seem natural as the discriminator fails to determine encoded images from natural images.

Due to the combined loss functions and their constraints of IDL $L_I$, adversarial Loss $L_G$ and noise addition, the encoder is unable to encode in low-frequency regions. The watermark is spread across multiple high frequencies and spatial locations, making it hard to spot and remove. This trait of HiDDeN is considered one of its strengths. However, it also makes it predictable as HiDDeN always hides information in the frequency domains' higher regions. This is HiDDeNs common signature across all WM images. UnMarker uses this common feature to always distort these frequency regions that are usually beyond the visible spectrum. UnMarker can attack these regions aggressively without distorting the image perceptually. Hence, the robustness and invisibility of HiDDeN also highlight their spectral vulnerability. This fundamental weakness in HiDDeN also raises questions about deep-learning-based watermarking schemes after the development of UnMarker.

\subsection{{StegaStamp}}
StegaStamp enhances the structural foundations of HiDDeN by extending its robustness properties from digital to also physical robustness of real-world print camera distortions. The working mechanism of StegaStamp is shown in Figure \ref{fig:stega_overview}. Therefore, the objective of StegaStamp remains the same, with a further extension whereby the decoder can detect the encoder's embedding even after the photo is printed out and rephotographed.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/Stega.png}
    \caption{Working mechanism of StegaStamp. Source: adapted from \cite{tancik2020stegastamp}.}
    \label{fig:stega_overview}
\end{figure}

\subsubsection{Encoder-decoder and detector networks}
StegaStamp uses a similar Encoder-Decoder to HiDDeN, with some added components key to real-world transformations. Between the Encoder and Decoder, a Spatial Transformer Network (STN) is used to remove geometric distortions. A localizer network is also used. Furthermore, the distortion module is extended to include brightness, colour, Gaussian blur and perspective distortions to mimic camera-based distortions. The method also introduces LPIPS to watermarking and adds a geometric reconstruction loss. 

In the cover image, the message is embedded as a small perturbation $\Delta \mathbf{x}$ as shown here: $\tilde{\mathbf{x}} = \mathbf{x} + \Delta \mathbf{x}$. StegaStamp replaces the standard CNN encoder with a U-Net architecture to preserve spatial features. Furthermore, it converts $M_{in}$ to a spatial tensor with spatial transformation before concatenation. This enables the encoder’s ability to embed across both spatial and frequency domains.

Additionally, StegaStamp requires a detection network in case images captured by the camera are scaled, rotated, or warped. The detector is based on BiSeNet (Bilateral Segmentation Network) and aligns the image to decoders expected input. The BiSeNet is trained to localize regions that likely contain a watermark. The detector operates as a semantic segmentation and provides a binary mask output on top of the image that highlights high-potential watermarked regions known as candidate regions. 

The decoder $D$ has the same objective as it did in HiDDeN and has a similar CNN structure. StegaStamp uses two stage geometric correction. Firstly, perspective transform (homography) is then applied on these candidate regions to make them decodable. Therefore, printed or on-screen images that have watermarks can be detected without knowing their exact locations. Afterwards, the Spatial Transformer Network (STN) is applied to the input of the decoder. 
 
The STN further refines alignment and makes corrections on geometric mistakes using homography.
STN is trained alongside the CNN. The STN warps input back to a reference frame. This enables the decoder to learn spatial transformations and makes $D$ robust to perspective changes and mild rotations. Similar to HiDDeN, the corrected image is then passed through convolutions and fully connected layers and finally passed through a sigmoid function to retrieve the $M_{out}$.


This combined detector–STN–decoder path allows StegaStamp to retrieve watermarks from printed or on-screen images without requiring prior knowledge of their exact position, scale, or orientation.
The StegaStamp decoding process follows the pipeline shown below. 

\noindent\resizebox{\linewidth}{!}{%
$I_{\text{photo}} \;\rightarrow\; \text{BiSeNet Detector} \;\rightarrow\; \text{Homography Rectification} \;\rightarrow\; \text{STN Alignment} \;\rightarrow\; \text{Decoder} \;\rightarrow\; \hat{m}$
}



\subsubsection{Critic network and adversarial loss}
In contrast to HiDDeN, StegaStamp incorporates a \textit{critic network} to enforce adversarial stealth. The critic plays a similar and is trained using a Wasserstein GAN loss with gradient penalty instead of binary cross-entropy. The critic in StegaStamp is trained using a Wasserstein loss in Equation \ref{eq:wgan_gp}. Here, $C_{\psi}$ is the critic network with parameters $\psi$, and $\mathbf{x}$ and $\tilde{\mathbf{x}}$ be the cover and encoded images, respectively. $\hat{\mathbf{x}}$ is a random interpolation between $\mathbf{x}$ and $\tilde{\mathbf{x}}$, and $\lambda_{GP}$ is the gradient penalty weight.

\begin{equation}
    \mathcal{L}_{\text{critic}} =
    \mathbb{E}[C_{\psi}(\tilde{\mathbf{x}})] -
    \mathbb{E}[C_{\psi}(\mathbf{x})] +
    \lambda_{GP} \, \mathbb{E}[(\|\nabla_{\hat{\mathbf{x}}} C_{\psi}(\hat{\mathbf{x}})\|_2 - 1)^2],
    \label{eq:wgan_gp}
\end{equation}

The critic network uses convolution layers followed by a global average pooling layer to reduce spatial dimensions, and a fully connected layer produces scalar outputs. This avoids the vanishing gradients and leads to smoother optimization of the encoder.

The encoder is simultaneously trained to fool the critic using the adversarial loss. Minimizing $\mathcal{L}_C$ encourages $E$ to generate encoded images that are indistinguishable to the critic.

$C_{\psi}$ captures a continuous statistical distance between encoded and natural images. This pushes the encoder to embed messages without introducing subtle statistical artifacts. Thus, $\mathcal{L}_C$ acts as a learned, distribution-aware invisibility constraint and contributes to the total loss in Equation~\ref{eq:stegastamp_loss}.


\subsubsection{Loss functions}
\label{sec:stegastamp_loss}

StegaStamp uses the same structure as HiDDeN. The Message Reconstruction Loss $\mathcal{L}_M$ and image distortion loss $\mathcal{L}_I$ serve as the backbone. $\mathcal{L}_M$ uses the binary cross entropy between $M_{\text{in}}$ and $M_{\text{out}}$.
The Reconstruction Loss is the same MSE as in HiDDeN with an added spatial weighting as shown in Equation \ref{eq:stegastamp_weighted_mse}. Here $w(x, y)$ is the spatial mask that is maximum close to an object's center and minimum at the edges. This ensures that distortions are added to the center of objects as edges are more noticeable.

\begin{equation}
    \mathcal{L}_I =
    \sum_{x,y}
    w(x, y) \cdot
    \left(
        I_{\text{co}}(x, y) - I_{\text{en}}(x, y)
    \right)^2,
    \label{eq:stegastamp_weighted_mse}
\end{equation}

A key weakness of HiDDeN is that the perceptual MSE used still allowed some noticeable perceptual perturbations in the image. StegaStamp tackles that by introducing LPIPS $\mathcal{L}_P$ to its embedding. LPIPS is discussed in Mathematical Basics and compares $\mathbf{x}$ and $\tilde{\mathbf{x}}$ from feature maps of convolutional layers. The feature maps represent edges and textures and LPIPS ensures embeddings are hard to detect by CNNs.


The discriminator in HiDDeN detects whether an image is watermarked or a cover image. StegaStamp makes a critical improvement in this section by introducing the Adversarial Loss $\mathcal{L}_C$ through a critic learned network. The critic loss is shown in Equation \ref{eq:stegastamp_critic_loss}. Here, $f_{\psi}$ is the critic network. The encoder minimizes this loss $\mathcal{L}_C$ so that the encoded image $I_{\text{en}}$ and cover image $I_{\text{co}}$ are indistinguishable. This makes the StegaStamp stronger than HiDDeN as it not only hides embedding from human eyes but also does not embed with patterns that CNNs can detect.

\begin{equation}
\mathcal{L_C} = -\mathbb{E}[f{\psi}(I_{\text{en}})] + \mathbb{E}[f_{\psi}(I_{\text{co}})],
\label{eq:stegastamp_critic_loss}
\end{equation}

The overall objective of StegaStamp is a weighted sum similar to HiDDen as shown in Equation \ref{eq:stegastamp_loss}. Here, $\lambda_M$, $\lambda_R$, $\lambda_P$, and $\lambda_C$ are the Lagrangian soft constraints that control the trade-off between robustness and imperceptibility.
\begin{equation}
    \mathcal{L}_{\text{total}} =
    \lambda_M \mathcal{L}_M +
    \lambda_R \mathcal{L}_R +
    \lambda_P \mathcal{L}_P +
    \lambda_C \mathcal{L}_C,
    \label{eq:stegastamp_loss}
\end{equation}
\noindent where:
\begin{itemize}
\item $\mathcal{L}_M$ controls accuracy of decoding of $M_{in}$.
\item $\mathcal{L}_R$ pushes the values of the watermarked image pixels close to the values of the original image pixels.
\item $\mathcal{L}_P$ is LPIPS, preserving visual similarity.
\item $\mathcal{L}_C$ forces encoder to embed watermark with high slealth.
\end{itemize}

\subsubsection{Differentiable noise layer}
The noise layer from HiDDeN focused on digital distortions. StegaStamp builds on it to include physical distortions in the noise layer. They use a differentiable distortion pipeline $\mathcal{T}$ as shown in Equation \ref{eq:stegastamp_pipeline}. The decoder $D$ receives a distorted cover image and is trained on that image.

\begin{equation}
\hat{\mathbf{m}} = D\big(\mathcal{T}(E(\mathbf{x}, \mathbf{m}))\big),
\label{eq:stegastamp_pipeline}
\end{equation}

$\mathcal{T}$ consists of differentiable transforms that simulate physical camera artifacts alongside digital ones shown in HiDDeN.

\begin{itemize}
\item \textit{Perspective Warp:} simulates camera angle/viewpoint changes by applying a homography.
\item \textit{Motion and Defocus Blur:} simulates convolution with motion (linear kernel) or defocus (Gaussian kernel) blur to mimic blur during photo captures.
\item \textit{Color Shift and Lighting:} simulates color shifts and brightness changes.
\item \textit{Additive Noise:} Gaussian noise ($\sigma \sim [0, 0.2]$) to simulate random noise noise.
\item \textit{Differentiable JPEG Compression:} simulates an approximate differentiable JPEG model for images.
\end{itemize}

\subsubsection{The output of StegaStamp}
An overview shows that StegaStamp and HiDDeN work very similarly to produce their watermarks. Each has an encoder $E$ to embed the message, a noise layer $N$ to make the watermarks robust, an adversarial training method to ensure that $E$ is hard to detect and finally the decoder $D$ that recovers the message. However, due to the slight changes in StegaStamp, a deeper dive finds that the results are vastly different for where the watermarks are embedded. 

As mentioned earlier, constraints ensured HiDDeN embeddings are mostly engraved in the high-frequency zones. Despite using a similar architecture, StegaStamp needs robustness to physical distortions. Physical distortions like printing and photo captures tend to impact these high-frequency zones first. For example, if a pixel intensity is changed by HiDDeN to embed, that may not be captured by a photo reshot. Thus, the addition of a differentiable noise layer forces the Encoder to prefer mid-to-low-frequency regions for embedding. Furthermore, the critic network and its loss act as a perceptual discriminator that penalizes high-frequency patterns and textures embedded by HiDDeN. This further enforces smooth low-frequency embeddings. These constraints reduce visibility and strengthen robustness to physical distortions. 

Therefore, the decoder of HiDDeN and StegaStamp work opposite to one another. The HiDDeN decoder, after training, can only detect high-frequency similar inputs. Meanwhile, the StegaStamp decoder reads outputs that are smooth spatially. The photo capture and noise layer acts as low pass filters and high-frequency regions become non-viable for embedding. Therefore, the noise layers of HiDDeN and StegaStamp show that type of noise the encoder-decoder structure is trained upon decides where the watermark is embedded in the image. This information is used later on by UnMarker to remove these watermarks. These semantic watermarking schemes were considered the future in tackling deepfake contents until before UnMarker was developed.

\subsection{The UnMarker}
The UnMarker is then introduced for removing these watermarks. UnMarker is a black-box optimization algorithm that can remove semantic and non-semantic watermarks without any prior knowledge of the watermarking scheme. This makes UnMarker unique and the authors considered it the first practical attack on semantic watermarks. For successful implementation, the UnMarker assumes the methods we deduced earlier in HiDDeN and StegaStamp. That is, for a watermark to be robust against distortions, they must be embedded in specific spectral amplitudes (frequency bands). They call these the universal spectral carrier. Therefore, these assumptions led to two types of watermarking schemes.

Non-semantic schemes do not influence the content of an image; they are invisible and focus on higher frequencies of the image.
Semantic schemes can influence the content of an image. Usually, they alter visible changes slightly, like the color and texture of the image and focus on low-frequency bands (i.e, StegaStamp). Based on the two above methods, UnMarker introduces two separate attacks: The non-semantic high-frequency attack and the semantic low-frequency attacks. Due to these attacks being separate technically, they are discussed in the latter two sections.

\subsubsection{Formal objective of UnMarker}

UnMarker targets the spectral carrier and disrupts the frequency components so that the decoder cannot decode the encoder embedding. Consequently, formally UnMarker works very similarly to above discussed watermarking schemes. 


Consider the images with watermarks $x'$ as spectral carriers $F_c$ that contain spectral (Fourier-domain) amplitudes as shown in Equation \ref{eq:Fc}. $F_c$ is the set of magnitudes of Fourier coefficients. $\lvert F_b \rvert$
 is their respective magnitudes for the frequency band $b$. $\mathcal{B}$ refers to the set of all the frequency bands.
\begin{equation}
F_c \;=\; \left\{\, \lvert F_b \rvert \;:\; b \in \mathcal{B} \right\},
\label{eq:Fc}
\end{equation}

The goal of UnMarker is to produce an output image $x_{\text{unmark}}$ that is perceptually close to the input watermarked image $x'$ such that the decoder fails to read the hidden message $m$. As discussed from LPIPS basics, here the visual difference $l_d$ refers to visual difference between the watermarked image $x'$ and the output image $x_{\text{unmark}}$ and they must be less than a certain threshold $t_{ld}$. Therefore, the objective is shown in Equation \ref{eq:unmarker_obj}. 

\begin{equation}
\begin{aligned}
x' \;\rightarrow\; x_{\text{unmark}} \\
l_d\!\left(x',x_{\text{unmark}}\right)\le t_{ld} \\
F_c\!\left(x_{\text{unmark}}\right)\neq F_c\!\left(x'\right) 
\end{aligned}
\label{eq:unmarker_obj}
\end{equation}



The watermarked image $x' = x + \Delta x$, where $x \in \mathbb{R}^{H \times W \times C}$ is the original image and $\Delta x$ is the encoded hidden message $m \in \{0,1\}^L$, the decoder $D$ aims to recover the message as:
\[
\hat{m} = D(x').
\]

Therefore, again, the same perceptual constraint is present. UnMarker uses the LPIPS constraint as shown in Equation \ref{eq:unmarker_lpips_constraint} to ensure visual distortion is minimal. $\varepsilon$ is the controlled variable that determines strictness.
\begin{equation}
\mathcal{L}_{\text{LPIPS}}(x_{\text{unmark}}, x') \leq \varepsilon,
\label{eq:unmarker_lpips_constraint}
\end{equation}


\subsubsection{Watermark removal optimization}
In the frequency spectrum, UnMarker disrupts the target frequencies where higher frequencies are most likely to be present. Therefore, the Fourier Transform of $x_{\text{unmark}}$ deviates from that of $x'$ in regions where $\mathcal{F}(\Delta x)$ is concentrated. Let $\mathcal{F}(\cdot)$ denote the Discrete Fourier Transform.
The UnMarker optimization problem is shown in Equation \ref{eq:unmarker_optim}. Here, $\mathcal{L}_{\text{spec}}$ is the maximized loss, and it calculates the difference in frequency amplitudes between the output unmarked image $x_{unmarked}$ and the watermarked image $x'$.
\begin{equation}
\resizebox{0.90\columnwidth}{!}{$\displaystyle
x_{\text{unmark}} = \arg\max_{x'} \;\mathcal{L}_{\text{spec}}(x_{unmark}, x') \quad \text{subject to} \quad \mathcal{L}_{\text{LPIPS}}(x_{unmark}, x') \leq \varepsilon,
$}
\label{eq:unmarker_optim}
\end{equation}





\subsection{{UnMarker’s Non-Semantic attack}}
Non-semantic watermarking schemes primarily inject watermarks in the global spectral amplitudes, which are associated with high frequencies. In high frequencies, mostly low-energy distribution or edges exist. For ensuring invisibility, the edges of the original images are used. Schemes are injected into these edges by adjusting pixel intensities. These schemes are typically very easy to hide.


\subsubsection{Direct Fourier loss}

The idea for a non-semantic attack is simple: UnMarker wants to maximize the difference between the watermarked image and the output image. As discussed in earlier sections, high frequencies are beyond the human visual spectrum and thus, Direct Fourier loss (DFL) is crucial. DFL calculates the frequency band-wise spectral differences and UnMarker aims to maximize this difference. To ensure that the visual difference is minimal, LPIPS is also minimized. Therefore, based on this information, the high frequency destruction of watermarks can be shown by the optimization algorithm shown in Equation \ref{eq:dfl}. Therefore, optimizing DFL as shown in Equation \ref{eq:dfl_max} maximizes the spectral amplitudes between the watermarked image and the output image. Hence, watermarks in the high-frequency bands are significantly changed and this makes the decoder fail to detect watermarks.


\subsubsection{Perceptual loss and norms}
UnMarker also needs to ensure that the images are visually similar. To do this, the authors considered DeepVGGLoss-LPIPS and LPIPSAlex as they represent human vision. Furthermore, they introduce an L2 norm that acts as a geometric boundary over the LPIPS. When LPIPS introduces too large a change in one direction, the norm forces it to consider other changes. Therefore, LPIPS limits perceptual deviation by penalizing any output when the LPIPS distance exceeds the threshold. The L2 norm $\lVert\rVert_2$ term limits the optimizer from concentrating distortion into only a few high-amplitude pixel changes. Therefore, even if LPIPS is satisfied, $\lVert\rVert_2$ ensures that there are no localized artifacts and perturbations are evenly distributed, which further enhances the visual quality of the image.


\subsubsection{Watermark removal procedure}
Therefore, based on the above information, the UnMarker objective is provided in Equation \ref{eq:unmarker_nonsemantic_opt}. The algorithm optimizes DFL while staying below the norm and LPIPS thresholds for the following inputs: watermarked image $x_w$, LPIPS loss $l_d$, LPIPS threshold $t_{ld}$, L2 norm $\lVert\rVert_2$ and L2 norm threshold as $t_2$

\begin{equation}
\begin{aligned}
x_{\text{um}} &= x_w + \delta^{\star} \\[2pt]
\delta^{\star} &= \arg\min_{\delta}\;
c_{\ell_p}\,ReLU\!(\ell_p(x_w+\delta,\,x_w))\\[-1pt]
&\quad\quad\quad\quad+ \,c_{\lVert\cdot\rVert_2}\,ReLU\!(x_w+\delta,\,x_w)
\;\;\\&\quad\quad\quad\quad - 
DFL(x_w+\delta,\,x_w) \\[2pt]
\end{aligned}
\label{eq:unmarker_nonsemantic_opt}
\end{equation}

 
\noindent\textbf{where}
\begin{equation*}
\resizebox{0.98\columnwidth}{!}{$
\begin{aligned}
x_w &:\ \text{input watermarked image},\\
x_{\text{um}} &:\ \text{output image},\\
\delta &:\ \text{perturbation optimized by UnMarker},\\
\delta^{\star} &:\ \text{optimal modifier},\\[2pt]
\ell_p(\cdot,\cdot) &:\ \text{LPIPS perceptual distance},\\
t_{\ell_p} &:\ \text{LPIPS threshold},\\
\lVert.\rVert_2 &:\ \ell_2 \text{ geometric constraint},\\
t_{\lVert\cdot\rVert_2} &:\ \ell_2 \text{ threshold},\\
\operatorname{ReLU}(z) &:\ =\max(0,z),\\
c_{\ell_p},\,c_{\lVert\cdot\rVert_2} &:\ \text{weights balancing LPIPS and }\ell_2\text{ hinge penalties},\\
F_c(\cdot) &:\ \text{spectral carrier (set of Fourier magnitudes across bands)},\\
\operatorname{DFL}(\cdot,\cdot) &:\ \text{Direct Fourier Loss (band-wise spectral magnitude disruption)}.
\end{aligned}
$}
\end{equation*}

Gradient ascent-based optimization is used to optimize the algorithm. The spectral term
\(-\mathrm{DFL}(x_w+\delta, x_w)\) is being maximized (hence it is negative) and is always active. During each iteration, the Fourier magnitude difference is pushed further to ensure stronger disruptions in the spectral carrier $F_c$. The LPIPS constraint term, $ReLU(\ell_p(x_w+\delta, x_w)$ is zero as long as the perceptual distance is less than the threshold \(t_{\ell_p}\). When \(\ell_p\) exceeds \(t_{\ell_p}\), the term is used to penalize the optimization hence pushing UnMarker towards a visually non-distorted solution. Finally,
the \(\ell_2\) constraint term is activated similarly when the geometric constant is violated. This ensures that perturbations of UnMarker are not too large in distinct locations, which may cause spikes. The thresholds can be set by the user. 



\subsection{{UnMarker’s semantic (low-freq) attack}}
Semantic watermarking schemes like StegaStamp embed their schemes into the low-frequency components of the image. Thus, they are woven into the textures of the image. Unlike high-frequency watermarks that manipulate single pixels, the low-frequency watermarks are required to add smooth transitions to make them invisible. The non-semantic attack is useless for these watermarking schemes. Therefore, the UnMarker proposed a new attack, the semantic attack. 

The semantic attack is completely different fundamentally. Knowing that low-frequency watermarks are woven into the image textures, the pixel-by-pixel manipulation of a non-semantic attack cannot remove the watermark and even if they succeed, large visual artifacts will be present. To succeed, groups of neighbouring pixels require simultaneous manipulation to ensure spatially smooth perturbations are added. To achieve this goal, the UnMarker introduces a novel adversarial filtering technique that is discussed later on in this section.

\subsubsection{How it works}
Generating low-frequency perturbations requires learned filters. Semantic attacks require smooth changes across the image that aggregate together to disrupt watermark embeddings. Filters are key for this. Filtering produces filtered pixels that are certain combinations of their neighbours and this results in spatially smooth changes with gradual intensity within the image. UnMarker uses this to its advantage and produces optimizable filters that can be changed based on the attack type. UnMarker's semantic attack takes the steps mentioned below to remove low-frequency watermarks.

The LPIPS guides the attack similarly to non-semantic attacks to ensure only non-critical areas are targeted. Therefore, this learned filtering approach is significantly more effective than random noise addition of non-semantic attacks for removing low-frequency watermarks.

\subsubsection{Parameterized filter}
For the above mentioned approach, UnMarker uses parameterized filters. That is, for each pixel \((i,j)\) in the image \(I\in\mathbb{R}^{M\times N\times C}\), an optimizable convolutional kernel \(K_{i,j}\in\mathbb{R}^{R\times R}\) of size \(R\times R\) is defined. This forms a set of filters \(K^{\star}=\{K_{i,j}\}_{i,j}\) that covers the whole image. The weights for each kernel is then adjusted based on the attack optimization during training. A color kernel \(C^{i,j}_{I_r,\sigma_c}\) is used to ensure that unnatural distortions are not created within the image to produce the kernel tensor \(\big[V_{R,K^{\star},\sigma_c}\big]_{i,j}\) for each pixel.

Therefore, the optimized filter can be shown in Equation \ref{eq:optimizable_filter}. The per-pixel tensors are shown in Equation \ref{eq:effective_kernel_tensor}. A guidance kernel 


\begin{equation}
\forall I:\quad
\mathrm{OF}_{K^{\star},R,\sigma_c}(I)
\;=\;
\sum_{m,n}\;
\mathrm{PE}^{M\times N}(I)\;\odot\;V_{R,K^{\star},\sigma_c},
\label{eq:optimizable_filter}
\end{equation}

\begin{equation}
\Big[V_{R,K^{\star},\sigma_c}\Big]_{i,j}
\;=\;
K_{i,j}\;\odot\;C^{i,j}_{I_r,\sigma_c}.
\label{eq:effective_kernel_tensor}
\end{equation}


The semantic attack stacks optimizable filters
sequentially to learn per-pixel kernels $\{K_t^{\star}\}_{t=1}^{T}$. The set of $K_t^{\star}$ contains $K^{t}_{i,j}$ for each pixel, which varies based on the image location. The color kernels \(C^{i,j}_{I_r,\sigma_c}\)
are computed from the watermarked image $x_w$ for applying geometric limitations in the optimization. Each filter layer $t$ has a unique geometry and parameter $\sigma_c^{t}$ that enables targeting various low-frequency regions where watermarks may be embedded. UnMarker uses these learned filter
stacks to distribute perturbations across a neighborhood (neighbouring pixels) via convolution, ensuring smooth and low-frequency changes. This is shown in detail in Equation \ref{eq:of_composition} and \ref{eq:adversarial_filtering}.


\begin{equation}
\widehat{\mathrm{OF}}^{(T)}
\;\triangleq\;
\mathrm{OF}^{1}_{K_1^{\star},\,x_w,\,\sigma_c^{1}}
\circ
\mathrm{OF}^{2}_{K_2^{\star},\,x_w,\,\sigma_c^{2}}
\circ \cdots \circ
\mathrm{OF}^{T}_{K_T^{\star},\,x_w,\,\sigma_c^{T}},
\label{eq:of_composition}
\end{equation}

where $\{\mathrm{OF}^{t}_{K_t^{\star},\,x_w,\,\sigma_c^{t}}\}_{t\in[[T]]}$ denotes a sequence of $T$ optimizable
filters. $\ell_d$ is the perceptual similarity loss based on LPIPS with
threshold $t_{\ell_d}$. Consider $\ell_F$ the low-frequency objective where watermarks are hidden. UnMarker optimizes and
then learns the filters using the kernel weights $\theta_{K_t^{\star}}$ with the additive modifier $\delta$ using Equation \ref{eq:adversarial_filtering}
\begin{equation}
\begin{aligned}
x_{nw}
&=
\arg\max_{\{\theta_{K_t^{\star}}\}_{t=1}^{T},\;\delta}\;
\ell_F\!\Big(x_w,\;\widehat{\mathrm{OF}}^{(T)}(x_w+\delta)\Big) \\
&\text{s.t.}\quad
\ell_d\!\Big(x_w,\;\widehat{\mathrm{OF}}^{(T)}(x_w+\delta)\Big)
\le t_{\ell_d}.
\end{aligned}
\label{eq:adversarial_filtering}
\end{equation}

\noindent\textbf{where}
\begin{equation*}
\resizebox{0.98\columnwidth}{!}{$
\begin{aligned}
x_w &:\ \text{input image},\\
x_{nw} &:\ \text{output image after semantic attack},\\
\widehat{\mathrm{OF}}^{(T)}(\cdot) &:\ \text{composition of $T$ optimizable filters (Eq.~\eqref{eq:of_composition})},\\
K_t^{\star} &:\ \text{set of per-pixel spectral kernels in layer } t,\ \text{i.e., } K_t^{\star}=\{K^{t}_{i,j}\}_{i,j},\\
\theta_{K_t^{\star}} &:\ \text{learnable weights that parameterize } K_t^{\star}\ \text{(optimized during the attack)},\\
\delta &:\ \text{additive modifier applied to } x_w \text{ before filtering},\\
\ell_F &:\ \text{low-frequency destruction objective},\\
\ell_d(\cdot,\cdot) &:\ \text{perceptual similarity loss constraint},\\
t_{\ell_d} &:\ \text{maximum perceptual loss threshold}.
\end{aligned}
$}
\end{equation*}




The maximization of Equation \ref{eq:adversarial_filtering} refers to passing the watermarked image $x_w$ with the additive modifier $\delta$ through networks and layers of optimizable filters $\widehat{\mathrm{OF}}^{(T)}(\cdot)$. This systematically distorts the targeted low-frequency regions and enforces perceptual similarity to ensure that changes within the image are limited to low-frequency regions.

$\delta$ in itself is useless for low-frequency disruption. However, optimizing $\delta$ across the filters spreads it across neighbouring pixels to create low-frequency noise that disrupts the watermark embeddings and eventually, watermark decoders fail to detect them. Although computationally expensive, this enables UnMarker massive flexibility and learn based on the structure of the watermark it is targetting to remove. Multiple convolutional layers can be stacked with kernels of different sizes to determine varying edges and structures with the watermark. UnMarker acts as a black box algorithm for semantic attacks. The filters being customizable themselves ensure that they can be trained and optimized for any low-frequency watermark removal.

\subsubsection{Filter regularization loss}
DFL introduced in non-semantic attacks maximized changes per pixel. However, that is not applicable for a semantic attack as changes are made throughout a neighborhood. To ensure visual similarity, regularization is required to ensure the image remains natural visually while still disrupting the watermarks.
Hence, the paper introduces Filter Regularization Loss (FRL).  The concept is that if a pixel tends towards being an outlier in its neighborhood, then it creates visual artifacts. Hence, each pixel is compared to its neighbours and large deviations are penalized. 

This operation is implemented with a median-filter operator $\mu_{\frac{1}{2}}$. For each pixel location $(i,j)$, the median is calculated within the kernel size $M_t \times N_t$ centered at $(i,j)$ as shown in Equation \ref{eq:frl_paper}. Here $M_t$ and $N_t$ denote the height
and width of the kernel in the $t^{\text{th}}$ filter layer. Maximizing FRL minimizes $\mathrm{FRL}_{t}(x)$. This enforces the pixel values to be as close to the median values as possible which leads to smooth patterns in the image and reduces visual artifacts.

\begin{equation}
\begin{aligned}
\forall x \in \mathbb{R}^{Q \times R}:\quad
\mathrm{FRL}(x)
&=
-
\sum_{t \in [[T]]}
\mathrm{FRL}_{t}(x),\\
\forall t \in [[T]]:\quad
\mathrm{FRL}_{t}(x)
&=
\left\lVert
x -
\mu_{\frac{1}{2}}(x)^{M_t \times N_t}
\right\rVert_{2}.
\end{aligned}
\label{eq:frl_paper}
\end{equation}


\subsubsection{Mean pool loss}
Semantic attacks use FRL in Eq.~\eqref{eq:frl_paper} for consistency in neighborhoods. However, FRL is limited only to local medians. 
In low-frequency watermarks, multiple pixels within a region are perturbed together which also changes the local medians in the same manner. The LPIPS constraints $\ell_d(\cdot,\cdot)$ already encourages preserving image content where possible. Therefore, even though FRL is satisfied, these local patches of watermarking schemes remain and the solution is not sub-optimal at best. 

To tackle these low-frequency regions, the authors introduce Mean Pool Loss (MPL). MPL compares patch averages within an $L\times P$ window instead of comparing pixels.
This partitions the image into neighborhoods of size $L\times P$. For two images, the MPL is shown in Equation \ref{eq:mpl_def}. This results in the unmarked image having different patch means compared to the watermarked image $x_wm$
$\mathrm{MP}_{L\times P}(\cdot)$ refers to the mean pooling term.

UnMarker maximizes $\mathrm{MPL}_{L\times P}(x_w, x)$ thereby forcing the output patch away from the watermarked image patch. This is a combination with FRL that plays a crucial role in destroying semantic watermarks. FRLs prevent visual artifacts and outliers, and MPL ensures there are patch-level changes in the output image. Thus, during optimiation the outlier pixels or neighborhoods (that carry watermarks) are pushed back towards median values (natural image values), hence removing watermark signatures.

\begin{equation}
\resizebox{0.90\columnwidth}{!}{$\displaystyle
\forall x,y \in \mathbb{R}^{Q\times R}:\quad
\mathrm{MPL}_{L\times P}(x,y)
=
\left\lVert
\mathrm{MP}_{L\times P}(x) - \mathrm{MP}_{L\times P}(y)
\right\rVert_{1}.
$}
\label{eq:mpl_def}
\end{equation}


Low-frequency objectives are spread throughout the image. Therefore, MPL operates on many patches. However, small windows (e.g., $1\times1$ or $3\times3$) make the loss similar to high-frequency loss as single pixel value changes will satisfy the optimization. Hence MPL uses $\mathrm{MPL}_{5\times5}$ pooling window to ensure that pixel noise while also controlling where these changes occur.

Furthermore, MPL can be satisfied by adding a constant offset in pixel values within the patches (physically, brightness changes in the image). However, this is not effective at removing watermark signatures. FRL acts as a regularizer in this case and ensures such extreme deviations do not occur within the image and the natural image structure remains intact. 

\subsubsection{The optimized output and objective}
Based on the above information, the object for the Unmarker's Semantic attack is shown in Equation \ref{eq:unmarker_semantic_final}. The objective consists of four main components. The primary objective is to maximize the two loss terms; MPL ($\mathrm{MPL}_{5\times 5}\!\big(x_w, x^{\widehat{\mathrm{OF}}^{(T)},\delta}_w\big)$) and FRL $\ (\lambda_{\mathrm{FRL}}\,\mathrm{FRL}\!\big(x^{\widehat{\mathrm{OF}}^{(T)},\delta}_w\big))$. Hence, they are negated in the equation. Furthermore, the norms and perceptual constraints as introduced in the non-semantic attack are also required. The perceptual constraint ($c_{\ell_{\mathrm{DVL}}}\,
\operatorname{ReLU}_{\ell_{\mathrm{DVL}}}\!\big(x_w, x^{\widehat{\mathrm{OF}}^{(T)},\delta}_w\big)$) is considered with a ReLU function to ensure that it is only non-zero when the perceptual loss is greater than the threshold $t_{\ell_{\mathrm{DVL}}}$. This enforces the LPIPS constraint and penalizes the objective when violated. Additionally, the $\ell_2$ regularization ($\lambda_{\lVert\cdot\rVert_2}\,
\big\lVert x^{\widehat{\mathrm{OF}}^{(T)},\delta}_w - x_w \big\rVert_2$) is also included to avoid drastic updates at each iteration, similar to a non-semantic attack.


\begin{equation}
\resizebox{0.90\columnwidth}{!}{$\displaystyle
\begin{aligned}
x_{nw} &=
\arg\min_{\{\theta_{K_t^{\star}}\}_{t=1}^{T},\,\delta}
\left[
\begin{aligned}
&c_{\ell_{\mathrm{DVL}}}\,
\operatorname{ReLU}_{\ell_{\mathrm{DVL}}}\!\big(x_w, x^{\widehat{\mathrm{OF}}^{(T)},\delta}_w\big)
+
\lambda_{\lVert\cdot\rVert_2}\,
\big\lVert x^{\widehat{\mathrm{OF}}^{(T)},\delta}_w - x_w \big\rVert_2 \\
&-\ \mathrm{MPL}_{5\times 5}\!\big(x_w, x^{\widehat{\mathrm{OF}}^{(T)},\delta}_w\big) -\ \lambda_{\mathrm{FRL}}\,
\mathrm{FRL}\!\big(x^{\widehat{\mathrm{OF}}^{(T)},\delta}_w\big)
\end{aligned}
\right] \\
x^{\widehat{\mathrm{OF}}^{(T)},\delta}_w &\equiv \widehat{\mathrm{OF}}^{(T)}(x_w+\delta)
\end{aligned}
$}
\label{eq:unmarker_semantic_final}
\end{equation}



\noindent\textbf{where}
\begin{equation*}
\resizebox{0.98\columnwidth}{!}{$
\begin{aligned}
x_w &:\ \text{input watermarked image} \\
x_{nw} &:\ \text{unmarker output after watermark removal} \\
\widehat{\mathrm{OF}}^{(T)}(\cdot) &:\ \text{composition of $T$ optimizable filters (Eq.~\ref{eq:of_composition})} \\
\{\theta_{K_t^{\star}}\}_{t=1}^{T} &:\ \text{learnable kernel weights for per-pixel kernels in each filter layer} \\
\delta &:\ \text{additive modifier of the input before filtering} \\
x^{\widehat{\mathrm{OF}}^{(T)},\delta}_w &:\ \text{output of the stacked filters applied to } x_w+\delta \\
\ell_{\mathrm{DVL}}(\cdot,\cdot) &:\ \text{perceptual loss} \\
\operatorname{ReLU}_{\ell_{\mathrm{DVL}}}(x_w,x) &:\ \max\!\big(0,\ \ell_{\mathrm{DVL}}(x_w,x)-t_{\ell_{\mathrm{DVL}}}\big) \\
t_{\ell_{\mathrm{DVL}}} &:\ \text{perceputal similarity threshold} \\
\mathrm{MPL}_{5\times 5}(\cdot,\cdot) &:\ \text{mean pool loss with a $5\times 5$ window (Eq.~\ref{eq:mpl_def})} \\
\mathrm{FRL}(\cdot) &:\ \text{filter regularization loss (Eq.~\ref{eq:frl_paper})} \\
c_{\ell_{\mathrm{DVL}}} &:\ \text{weight for the perceptual hinge term} \\
\lambda_{\lVert\cdot\rVert_2} &:\ \text{$\ell_2$ regularization weight to avoid drastic updates} \\
\lambda_{\mathrm{FRL}} &:\ \text{weight for FRL regularization} \\
\|\cdot\|_2 &:\ \ell_2 \text{ norm}
\end{aligned}
$}
\end{equation*}

This constrained optimization disrupts low-frequency watermarks. The output image's low-frequencies are removed with the UnMarker's additive. Hence, the structural patterns of the watermarking schemes are effectively not recognized by the decoder. Critically, the changes are distributed throughout the image while the image remains virtually the same. The results in the paper show that decoder detection rates drop to around 50\% from 100\% (random choice). UnMarker’s semantic attack is effective without any knowledge of the watermarking algorithm. The attack learns where to blur and where to preserve while systematically removing traces of watermark patterns purely on the watermarked image. 



